A Logical Interpretation of Asynchronous Multiparty Compatibility

Session types are types for specifying the protocols that communicating processes must follow in a concurrent system. When composing two or more well-typed processes, a session typing system must check whether such processes are multiparty compatible, a property that guarantees that all sent messages are eventually received and no deadlock ever occurs. Previous work has shown that duality and the more general notion of coherence are sufficient syntactic conditions for guaranteeing the multiparty compatibility property. In this paper, following a propositions-as-types fashion which relates session types to linear logic, we generalise coherence to forwarders. Forwarders are processes that act as middleware by forwarding messages according to a given protocol. Our main result shows that forwarders not only generalise coherence, but fully capture all well-typed multiparty compatible processes.

==> app-cll.tex <==
\mypar{Types.}
\begin{smallequation}\label{eq:types}
	\thl{A} ::=  \quad
	\thl{a}
	\: \mid\: \thl{a^\perp}
	\: \mid\: \thl{1}
	\: \mid\: \thl{\bot}
	\: \mid\: \thl{(A\tensor A)}
	\: \mid\: \thl{(A\parr A)}
	\: \mid\: \thl{(A\oplus A)}
	\: \mid\: \thl{(A\with A)}
	% \mid \thl{0}
	% \mid \thl{\top}
	% \thl{A^\perp} \mid
	\: \mid\: \thl{!A}
	\: \mid\: \thl{?A} 
\end{smallequation}
\mypar{Duality.}
\begin{smallequation*}
	\dual{(\dual{a})} = a
	\quad \dual\one=\perp
	\quad \dual{(A\tensor B)} = \dual A\parr\dual B
	\quad \dual {(A\oplus B)}=\dual A\with\dual B
	\quad \dual{(!A)} = ?\dual A
\end{smallequation*}

\mypar{Processes.} 
\begin{smallequation*}
  \begin{array}{l@{\quad}l@{\quad}l@{\qquad}l@{\quad}l@{\quad}l@{\qquad}l}
    \phl P,\phl Q ::= & \fwd xy          & \text{(link)}
    &
      \phl{\res {xy} (P\!\!\pp\!\! Q)} & \text{(parallel)}
    \\
                      & \wait x P & \text{(wait)}
    &
      \close x & \text{(close)}
    \\
                      & \recv xyP        & \text{(input)}
                
    &
      \send xyPQ       & \text{(output)}
    \\
    % & \recvtype xXP & \text{receive type}
    % &
    % \sendtype xAP & \text{send type}
    % \\
            & \Case xPQ        & \text{(choice)}
    & \inl xP          & \text{(left select)} \\
& & & \inr xP & \text{(right select)}
    \\
            & \client xyP & \text{(client request)}
    &
      \srv xyP & \text{(server accept)}
  
  \end{array}
\end{smallequation*}


\mypar{CP-typing.}
\begin{smallequation*}
    \begin{array}{c}
      \infer[\textsc{Ax}]
      {\phl{\fwd{x}{y}} \cll \phl x:\thl {a^\bot}, \phl y:\thl{a}}
      { }
      \qquad
      \infer[\bot]
      {\phl {\wait xP} \cll \thl \Delta, \phl x:\thl\bot}
      {\phl P \cll \thl\Delta}
      \qquad
      \infer[\one]
      {\phl{\close x} \cll \phl x: \thl\one}
      { }
      % \quad\qquad
      % \text{(no rule for $\zero$)}
      % \quad\qquad
      % \infer[\top]
      % {\phl{\emptyCase x\cll \thl{\Delta}}, \phl x:\thl\top}
      % { }    
      \\[1ex]
      \infer[\tensor]
      {
      \phl{\send xyPQ} 
      \cll 
      \thl{\Delta_1}, \thl{\Delta_2}, \phl x:\thl{A_1 \tensor A_2}
      }
      {
      \phl P 
      \cll 
      \thl{\Delta_1}, \phl y:\thl A_1
      & \phl Q 
        \cll 
        \thl \Delta_2, \phl x: \thl A_2
        }
        \qquad\qquad\qquad
        \infer[\parr]
        {\phl{\recv xyP} 
        \cll \thl{\Delta}, \phl x: \thl {A_1 \parr A_2}
        }       
        {\phl P \cll \thl{\Delta}, \phl y:\thl A_1, \phl x:\thl A_2}
      \\[1ex]
      \infer[\oplus_1]
      {\phl{\inl xP} \cll \thl\Delta, \phl x:\thl{A_1 \oplus A_2}}
      {\phl P \cll \thl\Delta, \phl x:\thl A_1}
      \qquad
      \infer[\oplus_2]
      {\phl{\inr xP} \cll \thl\Delta, \phl x:\thl{A_1 \oplus A_2}}
      {\phl P \cll \thl\Delta, \phl x:\thl A_2}
      \qquad
      \infer[\with]
      {\phl{\Case xPQ} \cll \thl \Delta, \phl x:\thl{A_1 \with A_2}}
      {\phl P \cll \thl\Delta, \phl x:\thl A_1 
      & 
        \phl Q \cll \thl\Delta, \phl x:\thl A_2}
      \\[1ex]
      \infer[?]
      {\phl{\client xyP} \cll \thl \Delta, \phl x:\thl {\query A}}
      {\phl P \cll \thl \Delta, \phl y:\thl A}
      \qquad\qquad
      \infer[!]
      {\phl{\srv xyP} \cll \,\thl{\query \Delta}, \phl x:\thl{\bang A}}
      {\phl P \cll \,\thl{\query \Delta}, \phl y:\thl A}
      \\[1ex]
      \infer[\textsc{Weaken}]
      {\phl P \cll \thl \Delta, \phl x:\thl{\query A}}
      {\phl P \cll \thl \Delta}
      % \\[1ex]
      % \infer[\exists]
      % {\phl{\sendtype xAP} \cll \thl \Delta, \phl x:\thl{\exists X.B}}
      % {\phl P \cll \thl \Delta, \phl x:\thl{B[A/X]}}
      % \ \quad
      % \infer[\forall]
      % {\phl{\recvtype xXP} \cll \thl\Delta, \phl x:\thl{\forall X.B}}
      % {\phl P \cll \thl\Delta, \phl x:\thl B & \thl X \notin \m{ftv}(\thl \Delta)}
                                                 \ \quad
                                                 \infer[\textsc{Contract}]
                                                 {\phl{P\{x/y, x/z\}} \cll \thl\Delta, \phl x:\thl{\query A}}
                                                 {\phl P \cll \thl\Delta, \phl y:\thl{\query A}, \phl
                                                 z:\thl{\query A}}
                                               % \\[1ex]
                                               % \qquad\qquad
                                               % \infer[\textsc{Cut}]
                                               % {\phl{\cpres{x}A{y}{A^\perp}(P
                                               % \pp Q)} \cll
                                               % \thl\Delta,\thl\Delta}
                                               % {\phl P \cll
                                               % \thl\Delta, \phl
                                               % x:\thl A & \phl Q
                                               % \cll \thl\Delta, \phl
                                               % y:\thl{\dual{A}}}
    \end{array}
  \end{smallequation*}


==> compatibility.tex <==
We now move to the describing the last feature of asynchronous
forwarders, i.e., the fact that they correspond to the notion of
multiparty compatibility. As mentioned in the early sections,
forwarders work as the fabric that describe the compatibility of the
processes that are being composed in an \tsc{MCutF} rule. The notion
of compatibility has been studied in the context of communicating
automata and then adopted to multiparty session
types~\cite{malo,alceste}. Following the approach by Ghilezal et al.,
we adopt the definition of multiparty compatibility to our typed
contexts.

In order to do so, we give a definition of reductions over a context
$\Delta$:
%
\begin{definition}[Context Reduction]
  The reduction $\Rightarrow$ over a forwarder context $\Gamma$ is
  inductively defined by the following rules, with $\alpha$ being
  either $???$ or $???$:
  \begin{displaymath}
    \begin{array}{lll}
      \infer[\tsc{E-Rcv}]
      {\Delta, \dbr{\Psi}\pairQ x{A\parr^y B}
      }
      {
      }
      &
        \infer[blah]
        {
        }
        {
        }
      \\\\
      \infer[blah]
      {
      }
      {
      }
      &
        \infer[blah]
        {
        }
        {
        }
    \end{array}
  \end{displaymath}
\end{definition}



\begin{definition}[Multiparty Compatibility]
  blah
\end{definition}


%
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> cutadm.tex <==
\subsection{General distribution and substitution}

\mypar{Distribution}

%We consider three cases, depending on if the element is a queued message $\br[d]{\pairQ bB}$, a branch $\br[d]{\Left}$, or a session $\br[d]{\Query}$, and define the corresponding distribution rule parameterized by connectives $\mathbf{CO} \bnfas \tensor \bnfalt \oplus \bnfalt ?$, and
%queues $\mathbf{Q} \bnfas {\pairQ bB} \bnfalt {\Left} \bnfalt {\Query}$. 
%
%$$
%\left\{
%\begin{array}{rcl}
%	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\mathbf{CO}^\bhl{\bm x}}} & \rhd & \br[d]{\mathbf{Q}}\dbr{\Psi_1}\pairQ{x}{A}
%	\\
%	\Gamma_2, \dbr{\Psi_{1c}}\bullet\dbr{\Psi_c}\pairQ{c}{C}& \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
%\end{array}
%\right\}
%\xrightarrow{\br[d]{\mathbf{Q}}\circ \phl{c}}_{\mathsf{distr}}
%$$
%
%$$
%\left\{
%\begin{array}{rcl}
%	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\mathbf{CO}^\bhl{\bm c}}} & \rhd & \dbr{\Psi_1}\pairQ{x}{A}\\
%	\Gamma_2, \dbr{\Psi_{1c}}\br[d]{\mathbf{Q}}\bullet\dbr{\Psi_c}\pairQ{c}{C} & \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
%\end{array}
%\right\}
%$$
%\noindent
%where the  $\mathbf{CO}^x$ refers to the leftmost occurence of a $\mathbf{CO}$ labelled with $x$ in $D$.

Multiplicatives with gathering
\[
		\left\{
		\begin{array}{l}
			\Gamma_1, \dbr{\Psi_{2z}} \bullet \dbr{\Psi_z} \pairQ
			z{B\{\tensor^\phl{\tilde vx}\}}
			\rhd
			\br[\phl z]{\{\Delta_i\}_i}\dbr{\Psi_1}\pairQ xA
			\\
			\Gamma_2, \big\{
			\dbr{\Psi_{1c_i}} \bullet \dbr{\Psi_{c_i}} \pairQ
			{c_i}{C_i}  \big\}_i
			\rhd
			\dbr{\Psi_2}\pairQ y{\dual A}
		\end{array}
		\right\}
		\xrightarrow{}_{\mathsf{distr}} %[^{\phl z}\{\Delta_i\}_i]\circ \{c_i\}_i
\]
\[
		\left\{
		\begin{array}{l}
			\Gamma_1, \dbr{\Psi_{2z}} \bullet \dbr{\Psi_z} \pairQ
			z{B\{\tensor^\phl{\tilde v\tilde c}\}}
			\rhd
			\dbr{\Psi_1}\pairQ xA
			\\
			\Gamma_2, \big\{
			\dbr{\Psi_{1c_i}}  \br[\phl z]{\Delta_i}\bullet \dbr{\Psi_{c_i}} \pairQ
			{c_i}{C_i}  \big\}_i
			\rhd
			\dbr{\Psi_2}\pairQ y{\dual A}
		\end{array}
		\right\}
\]

Additives


$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\oplus^{\bhl{\bm x}}}} & \rhd & \br[d]{\Left}\dbr{\Psi_1}\phl x: \thl A \\
	\Gamma_2, \dbr{\Psi_{1c}}\bullet\dbr{\Psi_c}\pairQ{c}{D} & \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
\xrightarrow{}_{\mathsf{distr}} %\br[d]{\Left}\circ \phl{c}
$$

$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D}\{\oplus^\bhl{\bm c}\} & \rhd &\dbr{\Psi_1}\pairQ{x}{A} \\
	\Gamma_2, \dbr{\Psi_{1c}}\br[d]{\Left}\bullet\dbr{\Psi_c}\pairQ{c}{C} & \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
$$



Exponentials 

$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\query^{\bhl{\bm x}}}} & \rhd & \br[d]{\Query}\dbr{\Psi_1}\phl x: \thl A \\
	\Gamma_2, \dbr{\Psi_{1c}}\bullet\dbr{\Psi_c}\pairQ{c}{D} & \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
\xrightarrow{}_{\mathsf{distr}} %\br[d]{\Query}\circ \phl{c}
$$

$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D}\{\query^\bhl{\bm c}\} & \rhd &\dbr{\Psi_1}\pairQ{x}{A} \\
	\Gamma_2, \dbr{\Psi_{1c}}\br[d]{\Query}\bullet\dbr{\Psi_c}\pairQ{c}{C} & \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
$$





\mypar{Substitution}

%We capture the substitution in one rule based on the top level collective $F = A (\mathbf{CO})^{\bhl{\bm b}} B$ and
%its dual $F ^\perp = \dual A \mathbf{(\mathbf{CO}^\perp)}^{\bhl{\bm c}} \dual B$, which expresses that communication will commence between $x$ and $\bhl{\bm b}$, and $y$ and $\bhl{\bm c}$, respectively.  Note that we slightly abuse notation by writing $\mathbf{CO}^\perp$ for the dual connective of $\mathbf{CO}$.  Substitution progresses then in a rather straightforward way: Identify the type of channel $b$ ($x$) and the topmost element ($y$) in the queue for $c$ and then  record the newly established connection between $b$ and $c$ by replacing  $x$ by $c$ and $y$ by $b$.
%The deceptive simple idea is capture by the following rule.
%
%$$
%\left\{
%\begin{array}{rcl}
%	\Gamma_1, \dbr{\Psi_b}\pairQ{b}{C\ctx{\mathbf{(\mathbf{CO}^\perp)}^\bhl{\bm x}}} & \rhd & \pairQ{x}{A (\mathbf{CO})^{\bhl{\bm b}} B} \\
%	\Gamma_2, \br[\bhl{\bm y}] {\mathbf{Q}}\dbr{\Psi_c}\pairQ{c}{D} & \rhd &
%	\pairQ{y}{\dual A \mathbf{(\mathbf{CO}^\perp)}^{\bhl{\bm c}} \dual B} \\
%	\text{or } \Gamma_2, \dbr{\Psi'_c}\pairQ{c}{D\ctx{(\mathbf{CO})^\bhl{\bm y}}} && (y \not\in\dbr{\Psi'_c})
%\end{array}
%\right\}
%\xrightarrow{}_{\mathsf{subst}} %\br[]{}\circ c
%$$
%$$
%\left\{
%\begin{array}{rcl}
%	\Gamma_1, \dbr{\Psi_b}\pairQ{b}{C\ctx{\mathbf{(\mathbf{CO}^\perp)}^\bhl{\bm c}}} & \rhd & \pairQ{x}{B} \\
%	\Gamma_2, \br[\bhl{\bm b}]{\mathbf{Q}}\dbr{\Psi_c}\pairQ{c}{D} & \rhd &
%	\phl y: \thl {B^\perp} \\
%	\text{or } \Gamma_2,  \dbr{\Psi'_c}\pairQ{c}{D\ctx{(\mathbf{CO})^\bhl{\bm b}}}
%\end{array}
%\right\}
%$$

Multiplicatives with gathering
\[
		\left\{
		\begin{array}{lcl}
			\Gamma_1, \dbr{\Psi_z}\pairQ
			z{E\{\tensor^{\phl{\tilde vx}}\}}
			&\rhd&
			\pairQ x{A\parr^{\phl z} B}
			\\
			\Gamma_2, \big\{\br[y]{\Delta_i}\dbr{\Psi_i}] \pairQ{c_i}{C_i}  \big\}_i,
			\big\{\dbr{\Psi_j}\pairQ{d_j}{D_j\ctx{\parr^{\phl y}}}\big\}_j
			&\rhd&
			\pairQ y{\dual A\tensor^\phl{\tilde c\tilde d}\dual B}
		\end{array}
		\right\}
		\xrightarrow{}_{\mathsf{subst}} %[^{\phl z}\{\Delta_i\}_i]\circ \{c_i\}_i
\]
\[	
\left\{
\begin{array}{lcl}
			\Gamma_1, \dbr{\Psi_z}\pairQ z{E\ctx\tensor^{\phl{\tilde v\tilde c\tilde d}}}
			&\rhd&
			\pairQ x{B}
			\\
			\Gamma_2, \big\{\br[z]{\Delta_i}\dbr{\Psi_i} \pairQ{c_i}{C_i}  \big\}_i,
			\big\{\dbr{\Psi_j}\pairQ{d_j}{D_j\{\parr^{\phl z}\}}\big\}_j
			&\rhd&
			\pairQ y{\dual B}
		\end{array}
		\right\}
\]

Additives
\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{x}}}\big\}_i
	&\rhd &
	\pairQ x{A \with^\phl{\tilde u} B}
	\\
	\Gamma_2, \br[y]{\Left}\dbr{\Psi_v} \phl v: \thl D
	&\rhd &
	\pairQ y{\dual A \oplus^\phl{v} \dual B}
\end{array}
\right\}
\longrightarrow_{\mathsf{subst}}
\left\{
\begin{array}{lcl}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{v}}}\big\}_i
	&\rhd &
	\pairQ x{B}
	\\
	\Gamma_2, \br[\tilde u]{\Left}\dbr{\Psi_v} \phl v: \thl D
	&\rhd &
	\pairQ y{\dual B}
\end{array}
\right\}
\]

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{x}}}\big\}_i
	&\rhd &
	\pairQ x{A \with^\phl{\tilde u} B}
	\\
	\Gamma_2, \dbr{\Psi_v} \phl v: \thl D\ctx{\with^\phl{y\tilde z}}
	&\rhd &
	\pairQ y{\dual A \oplus^\phl{v} \dual B}
\end{array}
\right\}
\longrightarrow_{\mathsf{subst}}
\left\{
\begin{array}{lcl}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{v}}}\big\}_i
	&\rhd &
	\pairQ x{B}
	\\
	\Gamma_2, \dbr{\Psi_v} \phl v: \thl D\ctx{\with^\phl{\tilde u\tilde z}}
	&\rhd &
	\pairQ y{\dual B}
\end{array}
\right\}
\]

Exponentials

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[i]{\dbr{\Psi_{u_i}}\pairQ{u_i}{B_i\ctx{\query^\phl{x}}}}
	&\rhd &
	\pairQ x{\bang^\phl{\tilde u} A} 
	\\
	\Gamma_2, \br[y]{\Query}\dbr{\Psi_z}\pairQ z{C}
	&\rhd &
	\pairQ y{\query^\phl{z} \dual A}
\end{array}
\right\}
\longrightarrow_{\mathsf{subst}}
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[i]{\dbr{\Psi_{u_i}}\pairQ{u_i}{B_i\ctx{\query^\phl{z} }}}
	&\rhd &
	\pairQ x{A} 
	\\
	\Gamma_2, \br[\tilde u]{\Query}\dbr{\Psi_z}\pairQ z{C}
	&\rhd &
	\pairQ y{\dual A}
\end{array}
\right\}
\]

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[i]{\dbr{\Psi_{u_i}}\pairQ{u_i}{B_i\ctx{\query^\phl{x}}}}
	&\rhd &
	\pairQ x{\bang^\phl{\tilde u} A} 
	\\
	\Gamma_2, \dbr{\Psi_z}\pairQ z{C\ctx{\bang^\phl{y}}}
	&\rhd &
	\pairQ y{\query^\phl{z} \dual A}
\end{array}
\right\}
\longrightarrow_{\mathsf{subst}}
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[i]{\dbr{\Psi_{u_i}}\pairQ{u_i}{B_i\ctx{\query^\phl{z} }}}
	&\rhd &
	\pairQ x{A} 
	\\
	\Gamma_2, \dbr{\Psi_z}\pairQ z{C\ctx{\bang^\phl{\tilde u}}}
	&\rhd &
	\pairQ y{\dual A}
\end{array}
\right\}
\]

\subsection{Cut-in-box lemmas}

%In contrast, the \cuttwo-rule defines communication between an active process and another that is enqueued elsewhere.
%
%\[
%    \infer[\cuttwo]
%    {\phl {\res{x\rhd w} (P\pp Q)}\seq\Gamma, [\Psi_1][^{\phl u}\pairQ z{\dual A}][\Psi_2]\pairQ y{B}}
%    {
%    \phl P\seq\pairQ z{\dual A}, \pairQ xA
%    &
%      \phl Q\seq\Gamma, [\Psi_1][^{\phl u}\pairQ w{\dual A}][\Psi_2]\pairQ y{B}
%    }
%\]


\begin{lemma} %[Admissibility of \cuttwo]
	\label{lem:cuttwo-adm}
  Let $\phl P\seq\Delta, \pairQ xA$ and
  $\phl Q\seq\Gamma, \dbr{\Psi_1}\br[\phl z]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ y{B}$ be derivable.
  Then, there exists $\phl R$ such that
  $\phl R\seq^\cut \Gamma, \dbr{\Psi_1}\br[\phl z]{\Delta}\dbr{\Psi_2}\pairQ y{B}$ is
  derivable with $\cut$ and $\mathtt{rank}(\phl{R}) = \mathtt{size}(A)$.
  %
  We denote this process as $\phl R = \phl{\res{x\rhd w}(P\pp Q)}$
\end{lemma}
\begin{proof}
By induction on the structure of $\phl Q$.
%
Because of the shape of its typing environment, $\phl Q$ cannot be of the shape $\fwd ab$ nor of the shape $\close a$.

Case $\phl Q = \send zvST$ and $\phl w\in \mathtt{fn}(\phl S)$.
%
Assume we have the following
\[
\infer[\tensor]{
	\phl{\send zvST} 
	\seq 
	\Gamma', \br[z]{\pairQ w{\dual A}}\dbr{\Psi_y}\pairQ yB, 
	\big\{\br[\phl z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_z}\pairQ z{D \tensor^\phl{y \tilde u} E}
}{
	\phl{S} \seq 
	\pairQ w{\dual A}, \big\{\Delta_i\big\}_i, \pairQ vD
	&
	\phl{T} \seq
	\Gamma', \dbr{\Psi_y}\pairQ yB, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_z}\pairQ zE
}
\]
%	where $\Gamma = \Gamma', \dbr{\Psi_u}\pairQ u{A \tensor^y C}$ and $\br[u]{...}\not\in\dbr{\Psi_1}$ -- so we can permeate $\br[u]{\pairQ{z}{\dual A}}$ to the top and we write $\dbr{\Psi_y}$ for $\dbr{\Psi_1}\dbr{\Psi_2}$.
%
We take $\phl R = \send zv{\res{xw}(P\pp S)}T$ and indeed $\mathtt{rank}(\phl R) = \mathtt{size}(A)$ as follows:
%	
\[
\infer[\tensor]{
	\send zv{\res{xw}(P\pp S)}T
	\seq
	\Gamma', \br[z]{\Delta}\dbr{\Psi_y}\pairQ yB, 
	\big\{\br[\phl z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_z}\pairQ z{D \tensor^\phl{y \tilde u} E}
}{	
	\infer[\cut]{
		\phl{\res{xw}(P\pp S)} \seq \Delta, \big\{\Delta_i\big\}_i, \pairQ vD
	}{
		\phl{P} \seq \Delta, \pairQ xA
		&
		\phl{S} \seq \pairQ w{\dual A}, \big\{\Delta_i\big\}_i,\pairQ vD
	}
	&
	\phl{T} \seq
	\Gamma', \dbr{\Psi_y}\pairQ yB, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_z}\pairQ zE
}
\]

This works because the labels in the left premiss are irrelevant to the conclusion, since the $\Delta$'s and the $D$ in the conclusion are not annotated (inside boxes and antecedent of $\tensor$ resp.).
%\todo{ needs to be explained.}

Case $\phl Q = \send zvST$ and $\phl w\in \mathtt{fn}(\phl T)$.
%
Assume we are in the following context %$\Gamma = \Gamma', \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}$.
\[
\infer[\tensor]{
	\send zvST
	\seq
	\Gamma', \br[z]{\Delta'}\dbr{\Psi_1}\br[z]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, 
	\big\{\br[z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i,  \dbr{\Psi_z}\pairQ z{C \tensor^\phl{y \tilde u} D}
}{
	\phl{S} \seq \Delta', \big\{\Delta_i\big\}_i,\pairQ vC
	&
	\phl T
	\seq
	\Gamma', \dbr{\Psi_1}\br[z]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i,  \dbr{\Psi_z}\pairQ z{D}
}
\]
%	
By applying the induction hypothesis to $\phl P$ and $\phl T$ (which indeed is a subprocess of $\phl Q$), we obtain $\phl{R_0}$ such that
$$\phl{R_0}\seq^\cut 
\Gamma', \dbr{\Psi_1}\br[z]{\Delta}\dbr{\Psi_2}\pairQ yB, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_z}\pairQ z{D}$$
and  $\mathtt{rank}(\phl{R_0}) = \mathtt{size}(A)$.
%
So we can take $\phl R = \send zvS{R_0}$
%	
and indeed, 
$$\phl R \seq^\cut \Gamma', \br[z]{\Delta'}\dbr{\Psi_1}\br[z]{\Delta}\dbr{\Psi_2}\pairQ yB, 
\big\{\br[z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i,  \dbr{\Psi_z}\pairQ z{C \tensor^\phl{y \tilde u} D}$$

When $\phl Q$ is of any other shape we can apply the induction hypothesis in a similar (or even simpler) way. \qed


%  \begin{itemize}
%  \item $\tensor$. We distinguish three cases: the case where the
%    $\tensor$ rule forwards the cut $\dual A$ and the ones where it
%    does not.
%    \begin{itemize}
%    \item {\em Case 1:} 
%    
%    Let $\mathcal D$ be the left premise of
%      \cuttwo\ and $\mathcal E_1$ and $\mathcal E_2$ be the proofs of
%      the two premise of rule $\tensor$ (for
%      $\phl{z} \not\in \Psi'_i, \Psi_1$):
%      \begin{itemize}
%       
%      \item $\mathcal D$: $\phl P\seq\Delta, \pairQ xA$
%      \item $\mathcal E_1$:
%        $ \phl {Q_1} \seq \big\{\Delta_i\big\}_i,\pairQ w{\dual A}, \pairQ {z'}{D_1}$ 
%      \item $\mathcal E_2$:
%        $\phl {Q_2} \seq \Gamma,\
%        \big\{[\Psi'_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\
%        [\Psi_1][\Psi_2]\pairQ y{B},\
%        [\Theta]\pairQ z{D_2}$
%      \item $\tensor \mathcal E_1\mathcal E_2$:
%        $\send z{z'}{Q_1}{Q_2} \!\seq\! \Gamma,\,
%        \big\{[\Psi'_i][^{\phl z}\Delta_i][\Psi''_i]\pairQ{r_i\!}{\!C_i}\big\}_i,\,
%        [\Psi_1][^{\phl z}\pairQ w{\dual A}][\Psi_2]\pairQ y{B},\,
%        [\Theta]\pairQ z{D_1\tensor^{\phl{\tilde r y}} D_2}$
%    \item 
%        $\cuttwo\ \mathcal D\ (\tensor\mathcal E_1\mathcal E_2)$:
%          $\phl {\res{x\!\rhd\! w} \big(P\!\pp\!
%          (\send z{z'}{Q_1}{Q_2})\big)} \!\seq\! \Gamma,\,
%        \big\{[\Psi'_i][^{\phl z}\Delta_i][\Psi''_i]\pairQ{r_i\!}{\! C_i}\big\}_i,\,
%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ y{B},\, [\Theta]\pairQ
%        z{D_1\tensor^{\phl{\tilde r y}} D_2}$
%      \end{itemize}
%  
%  	\[
%  	\infer[\cuttwo]{
%  		\phl {\res{x \rhd w} \big(P \pp \send z{z'}{Q_1}{Q_2} \big)}
%  		\seq
%  		\Gamma,
%  		\big\{\br[\phl z]{\Delta_i}\dbr{\Phi_i}\pairQ{r_i}{C_i}\big\}_i,
%  		\br[\phl z]{\Delta}\dbr{\Psi_2}\pairQ y{B},
%  		\dbr{\Theta}\pairQ z{D_1\tensor^{\phl{\tilde r y}} D_2}
%  	}{
%  		\phl P\seq\Delta, \pairQ xA
%  		&
%  		\infer[\tensor]{
%  			\send z{z'}{Q_1}{Q_2} 
%  			\seq
%  			\Gamma,
%  			\big\{\br[\phl z]{\Delta_i}\dbr{\Phi_i}]\pairQ{r_i}{C_i}\big\}_i,
%  			\br[\phl z]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ y{B},
%  			\dbr{\Theta}\pairQ z{D_1\tensor^{\phl{\tilde r y}} D_2}
%  		}{
%  			\phl {Q_1} \seq \big\{\Delta_i\big\}_i,\pairQ w{\dual A}, \pairQ {z'}{D_1}
%  			&
%  			\phl {Q_2} \seq \Gamma,
%  			\big\{\dbr{\Phi_i}\pairQ{r_i}{C_i}\big\}_i,
%  			\dbr{\Psi_2}\pairQ y{B},
%  			\dbr{\Theta}\pairQ z{D_2}
%  		}
%  	}
%  	\]
% 
%      By permuting and transforming $\cuttwo$ to an ordinary $\cut$,
%      we obtain:
%      \begin{itemize}
%      \item $\cut\ \mathcal D\ \mathcal E_1$:
%        $\phl {\res {xw}(P\pp Q_1)}\seq\Delta, \{\Delta_i\}_i,\pairQ {z'}{D_1}$
%      \item  
%      	$\tensor\ (\cut\ \mathcal D\mathcal E_1)\ \mathcal E_2$:
%        $\phl {\send z{z'\!}{\res {xw}(P\!\pp\! Q_1)}{Q_2}} \!\seq\! \Gamma,\,
%        \big\{[\Psi'_i][^{\phl z}\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\,
%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ y{B},\,
%        [\Theta]\pairQ z{D_1\tensor^{\phl{\tilde r y}} D_2}$        
%      \end{itemize}
%      
%      \[
%      \infer[\tensor]{
%      	\phl {\send z{z'\!}{\res {xw}(P\!\pp\! Q_1)}{Q_2}} 
%      	\seq
%      	\Gamma,
%      	\big\{\br[\phl z]{\Delta_i}\dbr{\Phi_i}\pairQ{r_i}{C_i}\big\}_i,
%      	\br[\phl z]{\Delta}\dbr{\Psi_2}\pairQ y{B},
%      	\dbr{\Theta}\pairQ z{D_1\tensor^{\phl{\tilde r y}} D_2}
%      	}{
%      		\infer[\cut]{      	
%      			\phl {\res {xw}P\pp Q_1}\seq\Delta, \{\Delta_i\}_i,\pairQ {z'}{D_1}
%      		}{
%      		\phl P\seq\Delta, \pairQ xA
%      		&
%      		\phl {Q_1} \seq \big\{\Delta_i\big\}_i,\pairQ w{\dual A}, \pairQ {z'}{D_1}
%      		}
%      	&
%      	\phl {Q_2} \seq \Gamma,
%      	\big\{\dbr{\Phi_i}\pairQ{r_i}{C_i}\big\}_i,
%      	\dbr{\Psi_2}\pairQ y{B},
%      	\dbr{\Theta}\pairQ z{D_2}
%      	}
%      \]
%      
%
%      
%    \item {\em Case 2:} Let $\mathcal D$ be the left premise of
%      \cuttwo\ and $\mathcal E_1$ and $\mathcal E_2$ be the proofs of
%      the two premise of rule $\tensor$ (for
%      $\phl{r} \not\in \Psi'_i$):
%
%      \begin{itemize}
%       
%      \item $\mathcal D$: $\phl P\seq\Delta, \pairQ xA$
%      \item $\mathcal E_1$:
%        $ \phl {Q_1} \seq \big\{\Delta_i\big\}_i, \pairQ {z'}{D_1}$
%      \item $\mathcal E_2$:
%        $\phl {Q_2} \seq \Gamma,\ 
%        \big\{[\Psi'_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\
%        [\Psi_1][^{\phl z}\pairQ{w}{\dual A}][\Psi_2]\pairQ y{B},\
%        [\Theta]\pairQ r{D_2}$
%      \item  $\tensor \mathcal D_1\mathcal D_2$:
%        $\send r{z'}{Q_1}{Q_2} \!\seq\! \Gamma,\,
%        \big\{[\Psi'_i][^{\phl r}\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\,
%        [\Psi_1][^{\phl z}\pairQ{w}{\dual A}][\Psi_2]\pairQ y{B},\,
%        [\Theta]\pairQ r{D_1\tensor^{\phl{\tilde r}} D_2}$
%      \item $\cuttwo\ \mathcal D\ (\tensor\mathcal E_1\mathcal E_2)$:
%        $\phl {\res{x \rhd w}\big(P\pp (\send r{z'}{Q_1}{Q_2})\big)} \!\seq\! \Gamma,\,
%        \big\{[\Psi'_i][^{\phl r}\Delta_i][\Psi''_i]\pairQ{r_i\!}{\! C_i}\big\}_i,\,
%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ {y\!}{\! B},\,
%        [\Theta]\pairQ r{D_1\tensor^{\phl{\tilde r}} D_2}$
%      \end{itemize}
%  
%  	\[
%  	\infer[\cuttwo]{
%  		\phl {\res{x\rhd w}\big(P\pp (\send u{z'}{Q_1}{Q_2})\big)} 
%  		\seq
%  		\Gamma,
%  		\big\{\br[\phl r]{\Delta_i}\dbr{\Psi_i}\pairQ{r_i}{C_i}\big\}_i,
%  		\br[\phl z]{\Delta}\dbr{\Psi}\pairQ {y}{B},
%  		\dbr{\Theta}\pairQ u{D_1\tensor^{\phl{\tilde r}} D_2}
%  		}{
%  		\phl P \seq \Delta, \pairQ xA
%  		&
%  		\infer[\tensor]{
%  			\send u{z'}{Q_1}{Q_2}
%  			\seq
%  			\Gamma,
%  			\big\{\br[\phl r]{\Delta_i}\dbr{\Psi_i}\pairQ{r_i}{C_i}\big\}_i,
%  			\br[\phl z]{\pairQ{w}{\dual A}}\dbr{\Psi}\pairQ y{B},
%  			\dbr{\Theta}\pairQ u{D_1\tensor^{\phl{\tilde r}} D_2}
%  			}{
%  			\phl {Q_1} \seq \big\{\Delta_i\big\}_i, \pairQ {z'}{D_1}
%  			&
%  			\phl {Q_2} \seq \Gamma,
%  			\big\{\dbr{\Psi_i}\pairQ{r_i}{C_i}\big\}_i,
%  			\br[\phl z]{\pairQ{w}{\dual A}}\dbr{\Psi}\pairQ y{B},
%  				\dbr{\Theta}\pairQ u{D_2}
%  			}
%  		}
%  	\]
%  
%      By permuting, we obtain:
%      \begin{itemize}
%      \item $\cuttwo\ \mathcal D\ \mathcal E_2$:
%        $\phl {\res{x\rhd w}(P\pp Q_2)} \seq \Gamma,\ 
%        \big\{[\Psi'_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\
%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ y{B},\
%        [\Theta]\pairQ r{D_2}$
%      \item $\tensor \mathcal E_1\ (\cut\ \mathcal D\mathcal E_2)$:
%        $\phl{\send r{z'}{Q_1}{\res{x\rhd w}(P\!\pp\! Q_2)}} \!\seq\! \Gamma,\,
%        \big\{[\Psi'_i][^{\phl r}\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\,
%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ y{B},\,
%        [\Theta]\pairQ {r\!}{\! D_1\tensor^{\phl{\tilde r}} D_2}$
%      \end{itemize}
%      
%      \[
%      \infer[\tensor]{
%      	\phl{\send r{z'}{Q_1}{\res{x\rhd w}(P\!\pp\! Q_2)}} 
%      	\seq 
%      	\Gamma,
%      	\big\{\br[\phl r]{\Delta_i}\dbr{\Psi_i}]\pairQ{r_i}{C_i}\big\}_i,
%      	\br[\phl z]{\Delta}\dbr{\Psi}\pairQ y{B},
%      	\dbr{\Theta}\pairQ {r}{D_1\tensor^{\phl{\tilde r}} D_2}
%      	}{
%      	\phl {Q_1} \seq \big\{\Delta_i\big\}_i, \pairQ {z'}{D_1}
%      	&
%      	\infer[\cuttwo]{
%      		\phl {\res{x\rhd w}(P\pp Q_2)} 
%      		\seq 
%      		\Gamma,
%      		\big\{\dbr{\Psi_i}\pairQ{r_i}{C_i}\big\}_i,
%      		\br[\phl z]{\Delta}\dbr{\Psi}\pairQ y{B},
%      		[\Theta]\pairQ r{D_2}
%      		}{
%      		 \phl P \seq \Delta, \pairQ xA
%      		  &
%      		  \phl {Q_2} \seq \Gamma,
%      		  \big\{\dbr{\Psi_i}\pairQ{r_i}{C_i}\big\}_i,
%      		  \br[\phl z]{\pairQ{w}{\dual A}}\dbr{\Psi}\pairQ y{B},
%      		  \dbr{\Theta}\pairQ r{D_2}
%      		}
%      	}
%      \]
%      
%       
%%    \item {\em Case 3:} Let $\phl{x} \not\in \Psi'_i$:
%%
%%      \begin{itemize}
%%       
%%      \item $\mathcal D$: $\phl P\seq\Delta, \pairQ xA$
%%      \item $\mathcal E_1$:
%%        $ \phl {Q_1} \seq \big\{\Delta_i\big\}_i, \pairQ {z'}{D_1}$. 
%%      \item $\mathcal E_2$:
%%        $\phl {Q_2} \seq \Gamma,\ 
%%        \big\{[\Psi'_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\
%%        [\Psi_1][^{\phl z}\pairQ w{\dual A}][\Psi_2]\pairQ y{B_2}$
%%      \item $\tensor \mathcal D_1\mathcal D_2$:
%%        $\send r{z'}{Q_1}{Q_2} \!\seq\! \Gamma,\,
%%        \big\{[\Psi'_i][^{\phl
%%          r}\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\,
%%        [\Psi_1][^{\phl z}\pairQ{w}{\dual A}][\Psi_2]\pairQ r{D_1\tensor^{\phl{\tilde r}} D_2}$
%%    \item $\cuttwo\ \mathcal D\ (\tensor\mathcal E_1\mathcal E_2)$:\\
%%        $\phl{\res{x\rhd w}\big(P\pp(\send r{z'}{Q_1}{Q_2})\big)} \!\seq\! \Gamma,\,
%%        \big\{[\Psi'_i][^{\phl
%%          r}\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\,
%%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ r{D_1\tensor^{\phl{\tilde r}} D_2}$
%%      \end{itemize}
%%      By permuting, we obtain:
%%      \begin{itemize}
%%      \item $\cuttwo\ \mathcal D\ \mathcal E_2$:
%%        $\phl {\res{x\rhd w}(P\pp Q_2)} \seq \Gamma,\ 
%%        \big\{[\Psi'_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\
%%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ y{B_2}$
%%
%%      \item $\tensor \mathcal E_1\ (\cut\ \mathcal D\mathcal E_2)$:\\
%%        $\phl{\send r{z'}{Q_1}{(\res{x\rhd w}(P\pp Q_2))}} \!\seq\! \Gamma,\,
%%        \big\{[\Psi'_i][^{\phl
%%          r}\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,\,
%%        [\Psi_1][^{\phl z}\Delta][\Psi_2]\pairQ
%%        r{D_1\tensor^{\phl{\tilde r}} D_2}$
%%
%%      \end{itemize}
%
%      
%    \end{itemize}
%
%    \bigbreak
%
%  \item $\parr$. In this case, we have two possibilities:
%    
%    \begin{itemize}
%    \item {\em Case 1}: Let $\mathcal D$ be the proof of the premise
%      of rule $\parr$.
%      \begin{itemize}
%      \item $\mathcal D$: $\phl P\seq\Delta, \pairQ xA$
%      \item $\mathcal E$:
%        $\phl R \seq \Gamma, [\Psi_1][^{\phl z}\pairQ w{\dual
%          A}][\Psi_2][^{\phl r} \pairQ wC]\pairQ yB$
%        
%      \item $\parr\mathcal E$:
%        $\phl{\recv yw{R}} \seq \Gamma, [\Psi_1][^{\phl z}\pairQ
%        w{\dual A}][\Psi_2]\pairQ y{C \parr^{\phl r} B}$
%
%      \item $\cuttwo\ \mathcal D\ (\parr\mathcal E)$:
%        $\phl{\res{x\rhd w}(P\pp \recv yw{R})} \seq \Gamma, [\Psi_1][^{\phl
%          z}\Delta][\Psi_2]\pairQ y{C \parr^{\phl r} B}$
%      \end{itemize}
%  
%  	
%  	\[
%  	\infer[\cuttwo]{
%  		\phl{\res{x\rhd w}(P\pp \recv yu{R})} \seq \Gamma, [\Psi_1][^{\phl
%  			z}\Delta][\Psi_2]\pairQ y{C \parr^{\phl r} B}
%  		}{	
%  		\phl P\seq\Delta, \pairQ xA
%  		&
%  		\infer[\parr]{
%  			\phl{\recv yu{R}} \seq \Gamma, [\Psi_1][^{\phl z}\pairQ
%  			w{\dual A}][\Psi_2]\pairQ y{C \parr^{\phl r} B}
%  			}{
%  			\phl R \seq \Gamma, [\Psi_1][^{\phl z}\pairQ w{\dual
%  				A}][\Psi_2][^{\phl r} \pairQ uC]\pairQ yB
%  			}
%  		}
%  	\]
%  
%  	
%      By permuting, we obtain:
%      \begin{itemize}
%      \item $\cuttwo\ \mathcal D\ \mathcal E$:
%        $\phl {\res{x\rhd w}(P\pp R)}\seq \Gamma, [\Psi_1][^{\phl z}{\Delta}][\Psi_2][^{\phl
%        r} \pairQ
%        wC]\pairQ yB$
%      \item $\parr (\cuttwo\ \mathcal D\ \mathcal E)$: 
%        $\recv yw{\res{x\rhd w}(P\pp R)}\seq \Gamma, [\Psi_1][^{\phl
%          z}\Delta][\Psi_2]\pairQ y{C\parr^{\phl r}B}$
%      \end{itemize}
%    \item {\em Case 2}: this case is similar to the previous one with
%      the difference that the cut formula $\dual A$ is in the queue of
%      another endpoint, rather than the queue of $\phl y$.
%    \end{itemize}
%  \end{itemize}
%
%
%
%    %   \phl{\send xy{P}Q} 
%    % \seq 
%    % \Gamma,
%    % \big\{[\Psi'_i][^x\Delta_i][\Psi''_i]\pairQ{r_i}{C_i}\big\}_i,
%    % [\Psi]\pairQ x{A \tensor^{\tilde z} B}
%    % }{
%    % & 
%    % &
%    %   {}
%    %   }


\end{proof}

In the binary case, it is possible to prove a stronger version  of this lemma where $\cut$ is not needed to construct $\phl{R}$, hence its rank is trivially null.

\begin{lemma} %[Admissibility of  \cuttwo]
	\label{lem:cuttwo-adm-simp}
	Let $\phl P\seq\pairQ z{\dual A}, \pairQ xA$ and
	$\phl Q\seq\Gamma, \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ y{B}$.
	Then, there exists $\phl R$ such that
	$\phl R\seq\Gamma, \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ y{B}$.
\end{lemma}

\begin{proof}
	By induction on the structure of $\phl Q$.
	
	Because of the shape of its typing environment, $\phl Q$ cannot be of the shape $\fwd ab$ nor of the shape $\close a$.
	
	When $\phl Q = \send uvST$ and $\phl w\in \mathtt{fn}(\phl S)$, we can take $\phl R = \send uxPT$.
	
	%	Indeed, assume $\Gamma = \Gamma', \dbr{\Psi_u}\pairQ u{A \tensor^y C}$ and $\br[u]{...}\not\in\dbr{\Psi_1}$ -- we therefore write $\dbr{\Psi_y}$ for $\dbr{\Psi_1}\dbr{\Psi_2}$.
	%	\[
	%	\infer[\cuttwo]{
	%		\phl {\res{x\rhd w} (P\pp \send uvST)}
	%		\seq
	%		\Gamma', \br[u]{\pairQ z{\dual A}}\dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ u{A \tensor^y C}
	%	}{
	%		\phl{P} \seq \pairQ z{\dual A}, \pairQ xA
	%		&
	%		\infer[\tensor]{
	%			\phl{\send uvST} 
	%			\seq 
	%			\Gamma', \br[u]{\pairQ w{\dual A}}\dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ u{A \tensor^y C}
	%		}{
	%			\phl{S} \seq \pairQ w{\dual A}, \pairQ vA
	%			&
	%			\phl{T} \seq
	%			\Gamma', \dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ uC
	%		}
	%	}
	%	\]
	%	\[
	%	\reducesto_\sigma\qquad
	%	\infer[\tensor]{
	%		\send uxPT
	%		\seq
	%		\Gamma', \br[u]{\pairQ z{\dual A}}\dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ u{A \tensor^y C}
	%	}{	
	%		\phl{P} \seq \pairQ z{\dual A}, \pairQ xA
	%		&
	%		\phl{T} \seq
	%		\Gamma', \dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ uC
	%	}
	%	\]
	
	When $\phl Q = \send uvST$ and $\phl w\in \mathtt{fn}(\phl T)$, by applying the induction hypothesis to $\phl P$ and $\phl T$ (subprocess of $\phl Q$), we obtain $\phl{R_0}$
	and take $\phl R = \send uvS{R_0}$.
	
	%	Indeed, assume $\Gamma = \Gamma', \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}$.
	%	
	%	\[
	%	\infer[\cuttwo]{
	%		\phl{\res{x\rhd w}(P \pp \send uvST)}
	%		\seq
	%		\Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}
	%	}{
	%		\phl{P} \seq \pairQ z{\dual A}, \pairQ xA
	%		&
	%		\infer[\tensor]{
	%			\send uvST
	%			\seq
	%			\Gamma', \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}
	%		}{
	%			\phl{S} \seq \pairQ f{\dual F}, \pairQ vF
	%			&
	%			\phl T
	%			\seq
	%			\Gamma', \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, \dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{C}
	%		}
	%	}
	%	\]
	%	\[
	%	\reducesto_\sigma
	%	\infer[\tensor]{
	%		\send uvS{\res{x\rhd w} (P\pp T)}
	%		\seq
	%		\Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}
	%	}{
	%		\phl{S} \seq \pairQ f{\dual F}, \pairQ vF
	%		&
	%		\infer[\cuttwo]{
	%			\phl{\res{x\rhd w} (P\pp T)}
	%			\seq
	%			\Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{C}
	%		}{
	%			\phl{P} \seq \pairQ z{\dual A}, \pairQ xA
	%			&
	%			\phl T
	%			\seq
	%			\Gamma', \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, \dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{C}
	%		}
	%	}
	%	\]
	
	When $\phl Q$ is of any other shape we can apply the induction hypothesis in a similar (simpler) way. 
\end{proof}

\subsection{Admissibility of Cut}


\begin{theorem} [Admissibility of Cut]
  Let $\phl P\seq\Gamma_1, \dbr{\Psi_1}\pairQ xA$ and
  $\phl Q\seq\Gamma_2, \dbr{\Psi_2}\pairQ y{A^\perp}$.
  For any $\Gamma$ such that
  $$\big\{\Gamma_1\rhd\dbr{\Psi_1}\pairQ xA,\ \Gamma_2\rhd\dbr{\Psi_2}\pairQ y{\dual
    A}\big\}\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma$$
  there exists $\phl R \seq \Gamma$.
\end{theorem}
\begin{proof}
	We proceed by lexicographic induction on the structures of $A$, $\phl P$ and $\phl Q$.
	That is, the induction hypothesis may be applied whenever 
	($i$) the rank of the cut gets smaller,
	%	 or ($ii$) the rank stays the same and a $\cuttwo$ is replaced by a $\cut$, 
	or ($ii$) the rank stays the same and the cut is applied to at least one smaller process while the other stays the same.
	

	
	\mypar{Axiom}
	
	\[
	\infer[\cut]{
		\phl{\res{xy}(\fwd zx \pp Q)}
		\seq
		\dbr{\Psi_2}\pairQ{z}{\dual a}, \Gamma_2[\phl z/ \phl y]
		}{
		\infer[\tsc{Ax}]{
			\fwd zx\seq\pairQ{z}{\dual a}, \pairQ xa
		}{}
		&
		\phl Q\seq \dbr{\Psi_2}\pairQ y{a^\perp}, \Gamma_2
		}
	\quad\reducesto_\beta\quad
	\phl{Q[z/y]}
	\seq
	\dbr{\Psi_2}\pairQ{z}{\dual a}, \Gamma_2[\phl z/ \phl y]
	\]
	
	\mypar{Units} 
	$$
	\infer[\textsc{Cut}]{
		\phl{\res {xy}(\close x \pp \wait {y}{Q}  )} \seq 
		\Gamma
	}{
		\infer[\one]{
			\close x \seq 
			\set[i]{\br[x]{\Star}\pairQ{u_i}{\cdot}}, \pairQ{x}{\one^\phl{\tilde u}}
		}{}
		&
		\infer[\bot]{
			\wait yQ \seq 
			\dbr{\Psi_2}\pairQ{y}{\bot^\phl{v}}, \Gamma_2,\dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{y\tilde{z}}}}
		}{
			\phl{Q} \seq
			\dbr{\Psi_2}\br[v]{\Star}\pairQ{y}{\cdot}, \Gamma_2,\dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{y\tilde{z}}}}
		}
	}
	$$
	$$
	\quad\reducesto_\beta\quad
	\infer[y \leadsto \tilde u]{
		\phl{Q^\mathsf{y \leadsto \tilde u}}
		\seq
		\set[i]{\dbr{\Psi_{u_i}}\br[v]{\Star}\pairQ{u_i}{\cdot}},
		\Gamma_2^\mathsf{y \leadsto \tilde u},\dbr{\Psi_c}\pairQ{v}{C^\mathsf{y \leadsto \tilde u}\ctx{\one^\phl{\tilde u\tilde{z}}}}
	}{
		\phl{Q} \seq \dbr{\Psi_2}\br[v]{\Star}\pairQ{y}{\cdot}, \Gamma_2, \dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{y\tilde{z}}}}
	}
	$$
	
	This is a special rule: It is not a uniform substitution replacing $\phl y$ by $\phl {\tilde{u}}$ but it reproduces the changes performed by the distribution of $\Psi$ over the $\phl{u_i}$s.
	%
	Because $\dbr\Psi$ is distributed from a terminated endpoint $\phl y$ to another list of endpoints in $\phl{\tilde u}$ that are also terminated, this rule is trivially admissible.
	
	
	$$
	\left\{
	\begin{array}{rcl}
		\set[i]{\br[x]{\Star}\pairQ{u_i}{\cdot}} & \rhd & \pairQ{x}{\one^{\tilde u}}\\
		\Gamma_2,\dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}} & \rhd & \dbr{\Psi}\pairQ{y}{\bot^v}
	\end{array}
	\right\}
	%	$$
	%	$$
	\xrightarrow{}_{\mathsf{distr}}^*
	\left\{
	\begin{array}{rcl}
		\set[i]{\dbr{\Psi_{u_i}}\br[x]{\Star}\pairQ{u_i}{\cdot}} & \rhd & \pairQ{x}{\one^{\tilde u}}\\
		\Gamma_2^\mathsf{y \leadsto \tilde u},\dbr{\Psi_c}\pairQ{v}{C^\mathsf{y \leadsto \tilde u}\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}} & \rhd & \pairQ{y}{\bot^v}
	\end{array}
	\right\}
	$$
	$$
	\xrightarrow{}_{\mathsf{subst}}
	\set[i]{\dbr{\Psi_{u_i}}\br[v]{\Star}\pairQ{u_i}{\cdot}},
	\Gamma_2^\mathsf{y \leadsto \tilde u},\dbr{\Psi_c}\pairQ{v}{C^\mathsf{y \leadsto \tilde u}\ctx{\one^\phl{\tilde{z_1}{\tilde u}\tilde{z_2}}}}
	= \Gamma
	$$  
	
	
	%	Knowing that the first step of the series of distribution looks like this:
	%	$$
	%	\left\{
	%	\begin{array}{rcl}
	%		\set[i\setminus k]{\bullet\br[x]{\Star}\pairQ{u_i}{\cdot}} , \bullet\br[x]{\Star}\pairQ{u_k}{\cdot}& \rhd & \pairQ{x}{\one^{\tilde u}}\\
	%		\Gamma_2', \dbr{\Psi_d}\pairQ{d}{D\ctx{\tensor^\phl{y}}}& \rhd & \br[d]{\pairQ{b}{B}}\dbr{\Psi'}\pairQ{y}{\bot^v}
	%	\end{array}
	%	\right\}
	%	\xrightarrow{}_{\mathsf{distr}} %\br[d]{\pairQ bB}\circ \phl{u_k}
	%	\left\{
	%	\begin{array}{rcl}
	%		\set[i]{\bullet\br[x]{\Star}\pairQ{u_i}{\cdot}}, \br[d]{\pairQ{b}{B}}\bullet\br[x]{\Star}\pairQ{u_k}{\cdot} & \rhd & \pairQ{x}{\one^{\tilde u}}\\
	%		\Gamma_2', \dbr{\Psi_d}\pairQ{d}{D\ctx{\tensor^\phl{u_k}}}& \rhd & \dbr{\Psi'}\pairQ{y}{\bot^v}
	%	\end{array}
	%	\right\}
	%	$$
	%	
	
	
	
	
	\mypar{Multiplicatives}
	$$
	\infer[\textsc{Cut}]{
		\phl{\res{xy}(\send xa{P}{Q} \pp \recv yc{R}) }
		\seq
		\Gamma
	}{
		\infer[\tensor]{
			\phl{\send xa{P}{Q}} 
			\seq 
			\Gamma_1,
			\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C},
			\dbr{\Psi_1}\pairQ x{A \tensor^\phl{u} B}
		}{
			\phl {P}
			\seq
			\pairQ{d}{\dual A},\pairQ aA
			& 
			\phl {Q} 
			\seq
			\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C}, \dbr{\Psi_1}\pairQ xB
		}
		&
		\infer[\parr]{
			\phl{\recv yc{R}} 
			\seq 
			\dbr{\Psi_2}\pairQ y{\dual A \parr^v \dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}
		}{
			\phl {R}
			\seq 
			\dbr{\Psi_2}\br[v]{\pairQ c{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}
		}
	}
	$$
	
	$$
	\quad\reducesto_\beta\quad
	\infer[\tsc{Cut}]{
		\phl {\res{xy} (Q\pp \res{a\rhd c} (P\pp R))}
		\seq
		\Gamma
	}{
		\phl {Q} 
		\seq
		\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C}, \dbr{\Psi_1}\pairQ xB
		&
		%		\infer[\tsc{Cut$_2$}]{
		\phl {\res{a\rhd c} (P\pp R)}
		\seq 
		\dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}
		%		}{
		%			\phl {P}
		%			\seq
		%			\pairQ{d}{\dual A},\pairQ aA
		%			&
		%			\phl {R}
		%			\seq 
		%			\Gamma_2, \dbr{\Psi_2}\br[v]{\pairQ c{\dual A}}\pairQ y{\dual B}
		%		}
	}
	$$
	
	By Lemma~\ref{lem:cuttwo-adm-simp}, we know that $\phl S \seq \dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}$, which gives us the right premiss above.
	%
	Then, the new $\cut$ (on $B$) is admissible by induction hypothesis on the rank as $\mathtt{size}(B) < \mathtt{size}(A \tensor^u B)$.
	
	$$
	\left\{
	\begin{array}{rcl}
		\Gamma_1,
		\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C} & \rhd & 
		\dbr{\Psi_1}\pairQ x{A \tensor^\phl{u} B}\\
		\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}} & \rhd &  \dbr{\Psi_2}\pairQ y{\dual A \parr^\phl{v} \dual B} 
	\end{array}
	\right\}
	%\xrightarrow{}_{\mathsf{distr}}^*
	%$$
	%
	%$$
	%\left\{
	%\begin{array}{rcl}
	%	\Gamma_1',
	%	\dbr{\Psi_{2e}}\bullet\dbr{\Psi_e}\pairQ{e}{E\ctx{\tensor^\phl{ x}}} & \rhd & 
	%	\br[e]{\pairQ fF}\dbr{\Psi_1'}\pairQ x{A \tensor^u B}\\
	%	\Gamma_2', \dbr{\Psi_{1g}}\bullet\dbr{\Psi_g}\pairQ{g}{G} & \rhd &  \dbr{\Psi_2'}\pairQ y{\dual A \parr^v \dual B} 
	%\end{array}
	%\right\}
	%$$
	%$$
	%\xrightarrow{\br[e]{\pairQ fF}\circ \phl{g}}_{\mathsf{distr}}
	%\left\{
	%\begin{array}{rcl}
	%	\Gamma_1',
	%	\dbr{\Psi_{2e}}\bullet\dbr{\Psi_e}\pairQ{e}{E\ctx{\tensor^\phl{g}}} & \rhd & 
	%	\dbr{\Psi_1'}\pairQ x{A \tensor^u B}\\
	%	\Gamma_2', \dbr{\Psi_{1g}}\br[e]{\pairQ fF}\bullet\dbr{\Psi_g}\pairQ{g}{G} & \rhd &  \dbr{\Psi_2'}\pairQ y{\dual A \parr^v \dual B} 
	%\end{array}
	%\right\}
	%$$
	%
	%$$
	\xrightarrow{}_{\mathsf{distr}}^*
	\left\{
	\begin{array}{rcl}
		\Gamma_1'',
		\dbr{\Psi_{2u}}\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
		\pairQ x{A \tensor^\phl{u} B}\\
		\Gamma_2'', \dbr{\Psi_{1v}}\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{y}}} & \rhd &  \pairQ y{\dual A \parr^\phl{v} \dual B} 
	\end{array}
	\right\}
	$$
	
	$$
	\xrightarrow{}_{\mathsf{subst}}
	\left\{
	\begin{array}{rcl}
		\Gamma_1'',
		\dbr{\Psi_{2u}}\br[v]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
		\pairQ x{B}\\
		\Gamma_2'', \dbr{\Psi_{1v}}\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{u}}} & \rhd &  \pairQ y{\dual B} 
	\end{array}
	\right\}
	\xrightarrow{}_{\mathsf{subst}}^*
	\Gamma
	$$
	
	On the other hand:
	$$
	\left\{
	\begin{array}{rcl}
		\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C} & \rhd &
		\dbr{\Psi_1}\pairQ x{B}\\
		\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}} & \rhd & \dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}
	\end{array}
	\right\}
	\xrightarrow{}_{\mathsf{distr}}^*
	\left\{
	\begin{array}{rcl}
		\Gamma_1'',
		\dbr{\Psi_{2u}}\bullet\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
		\pairQ x{B}\\
		\Gamma_2'', \dbr{\Psi_{1v}}\bullet\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{y}}} & \rhd &  \br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B} 
	\end{array}
	\right\}
	$$
	$$
	\xrightarrow{}_{\mathsf{distr}}
	\left\{
	\begin{array}{rcl}
		\Gamma_1'',
		\dbr{\Psi_{2u}}\br[v]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
		\pairQ x{B}\\
		\Gamma_2'', \dbr{\Psi_{1v}}\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{u}}} & \rhd &  \pairQ y{\dual B} 
	\end{array}
	\right\}
	\xrightarrow{}_{\mathsf{subst}}^*
	\Gamma
	$$
	
\mypar{Multiplicatives with gathering}

\[
\infer[\textsc{Cut}]{
	\phl{\res{xy}(\send xa{P}{Q} \pp \recv yc{R}) }
	\seq
	\Gamma
}{
	\infer[\tensor]{
		\phl{\send xa{P}{Q}} 
		\seq 
		\Gamma_1,
		\big\{\br[\phl x]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i,
		\dbr{\Psi_1}\pairQ x{A \tensor^\phl{\tilde u} B}
	}{
		\phl {P}
		\seq
		\big\{\Delta_i\big\}_i, \pairQ aA
		& 
		\phl {Q} 
		\seq
		\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_1}\pairQ xB
	}
	&
	\infer[\parr]{
		\phl{\recv yc{R}} 
		\seq 
		\dbr{\Psi_2}\pairQ y{\dual A \parr^v \dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}}
	}{
		\phl {R}
		\seq 
		\dbr{\Psi_2}\br[v]{\pairQ c{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}}
	}
}
\]

With $\Gamma$ being defined as one of the possible rewriting:
\[
\left\{
\begin{array}{ll}
	\Gamma_1,
	\big\{\br[\phl x]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i
	\rhd 
	\dbr{\Psi_1}\pairQ x{A \tensor^\phl{\tilde u} B}
	\\
	\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}} 
	\rhd 
	\dbr{\Psi_2}\pairQ y{\dual A \parr^\phl{v} \dual B}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}
\Gamma
\]

We want to reduce the cut as follows:
\[
\infer[\tsc{Cut}]{
	\phl {\res{xy} (Q\pp \res{a\rhd c} (P\pp R))}
	\seq
	\Gamma
}{
	\phl {Q} 
	\seq
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i, \dbr{\Psi_1}\pairQ xB
	&
	%		\infer[\tsc{Cut$_2$}]{
	\phl S 
	\seq 
	\dbr{\Psi_2}\br[v]{\big\{\Delta_i\big\}_i}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}}
	%		}{
	%			\phl {P}
	%			\seq
	%			\pairQ{d}{\dual A},\pairQ aA
	%			&
	%			\phl {R}
	%			\seq 
	%			\Gamma_2, \dbr{\Psi_2}\br[v]{\pairQ c{\dual A}}\pairQ y{\dual B}
	%		}
}
\]


By Lemma~\ref{lem:cuttwo-adm}, we know that $\phl S = \phl{\res{a\rhd c}(P\pp R)}$ exists, that 
$$\phl S \seq^\cut \dbr{\Psi_2}\br[v]{\big\{\Delta_i\big\}_i}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}}$$
and that its rank is equal to the size of $A$. 
%
By induction hypothesis any cut in the derivation of $\phl S$ is admissible as $\mathtt{rank}(\phl S) = \mathtt{size}(A) < \mathtt{size}(A \tensor^\phl{\tilde u} B)$.
%
That means in fact that 
$$\phl S \seq \dbr{\Psi_2}\br[v]{\big\{\Delta_i\big\}_i}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}}$$ 
without the need for cut, which gives us the right premiss.
%

Then, we need to check that we also get $\Gamma$ as conclusion, namely that we get 
%\todo{state this as lemma?}
\[
\left\{
\begin{array}{ll}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\big\}_i
	& \rhd 
	\dbr{\Psi_1}\pairQ xB
	\\
	\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y\tilde z}}}
	& \rhd 
	\dbr{\Psi_2}\br[v]{\big\{\Delta_i\big\}_i}\pairQ y{\dual B}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma
\]

Finally, the reduced $\cut$ (on $B$) is of course admissible by induction hypothesis on the rank as $\mathtt{size}(B) < \mathtt{size}(A \tensor^\phl{\tilde u} B)$.

\mypar{Additives}
$$
\infer[\tsc{Cut}]{
	\phl{\res{xy}(\Case{x}{P}{Q} \pp \inl yR )}
	\seq \Gamma
}{
	\infer[\with]{
		\Case{x}{P}{Q}
		\seq \Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{x}}}\big\}_i,
		\dbr{\Psi_1}\pairQ x{A \with^\phl{\tilde u} B}
	}{
		\phl {P}\seq \ldots,
		\dbr{\Psi_1}\br[\tilde u]{\Left}\pairQ xA
		&
		\phl {Q}\seq \ldots,
		\dbr{\Psi_1}\br[\tilde u]{\Right}\pairQ xB
	}
	&
	\infer[\oplus_l]{
		\inl yR \seq
		\dbr{\Psi_2}\pairQ y{\dual A \oplus^\phl{v} \dual B},
		\Gamma_2, \br[y]{\Left}\dbr{\Psi_v} \phl v: \thl D
	}{
		\phl R \seq
		\dbr{\Psi_2}\pairQ y{\dual A},
		\Gamma_2, \dbr{\Psi_v} \phl v: \thl D
	}
}
$$

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{x}}}\big\}_i
	&\rhd &
	\dbr{\Psi_1}\pairQ x{A \with^\phl{\tilde u} B}
	\\
	\Gamma_2, \br[y]{\Left}\dbr{\Psi_v} \phl v: \thl D
	&\rhd &
	\dbr{\Psi_2}\pairQ y{\dual A \oplus^\phl{v} \dual B}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\Gamma'_1, \big\{\dbr{\Psi_{2u_i}}\dbr{\Psi_{u_i}}\pairQ{u_i}{C'_i\ctx{\oplus^\phl{x}}}\big\}_i
	&\rhd &
	\pairQ x{A \with^\phl{\tilde u} B}
	\\
	\Gamma_2', \dbr{\Psi_{1 v}}\br[y]{\Left}\dbr{\Psi_v} \phl v: \thl D'
	&\rhd &
	\pairQ y{\dual A \oplus^\phl{v} \dual B}
\end{array}
\right\}
\]
\[
\longrightarrow_{\mathsf{subst}}
\left\{
\begin{array}{lcl}
	\Gamma'_1, \big\{\dbr{\Psi_{2u_i}}\dbr{\Psi_{u_i}}\pairQ{u_i}{C'_i\ctx{\oplus^\phl{v}}}\big\}_i
	&\rhd &
	\pairQ x{B}
	\\
	\Gamma_2', \dbr{\Psi_{1 v}}\br[\tilde u]{\Left}\dbr{\Psi_v} \phl v: \thl D'
	&\rhd &
	\pairQ y{\dual B}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{subst}}\Gamma
\]

$$
%\quad\reducesto_\beta\quad
\infer[\tsc{Cut}]{
	\phl{\res{xy}(P \pp R )}
	\seq \Gamma
}{
	\phl {P}\seq \Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{x}}}\big\}_i,
	\dbr{\Psi_1}\br[\tilde u]{\Left}\pairQ xA
	&
	\phl R \seq
	\dbr{\Psi_2}\pairQ y{\dual A},
	\Gamma_2, \dbr{\Psi_v} \phl v: \thl D
}
$$

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \big\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i\ctx{\oplus^\phl{x}}}\big\}_i
	&\rhd &
	\dbr{\Psi_1}\br[\tilde u]{\Left}\pairQ xA
	\\
	\Gamma_2, \dbr{\Psi_v} \phl v: \thl D
	&\rhd &
	\dbr{\Psi_2}\pairQ y{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\Gamma'_1, \big\{\dbr{\Psi_{2u_i}}\bullet\dbr{\Psi_{u_i}}\pairQ{u_i}{C'_i\ctx{\oplus^\phl{x}}}\big\}_i
	&\rhd &
	\br[\tilde u]{\Left}\pairQ xA
	\\
	\Gamma_2', \dbr{\Psi_{1 v}}\bullet\dbr{\Psi_v} \phl v: \thl D'
	&\rhd &
	\pairQ y{\dual A}
\end{array}
\right\}
\]
\[
\longrightarrow_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\Gamma'_1, \big\{\dbr{\Psi_{2u_i}}\dbr{\Psi_{u_i}}\pairQ{u_i}{C'_i\ctx{\oplus^\phl{v}}}\big\}_i
	&\rhd &
	\pairQ x{B}
	\\
	\Gamma_2', \dbr{\Psi_{1 v}}\br[\tilde u]{\Left}\dbr{\Psi_v} \phl v: \thl D'
	&\rhd &
	\pairQ y{\dual B}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{subst}}\Gamma
\]

\mypar{Exponentials}

$$
\infer[\cut]{
	\phl{\res{xy}(\srv xaP \pp \client ybQ )}
	\seq \Gamma %= \set[i]{\dbr{\Psi_{u_i}}\pairQ{u_i}{\query^z B_i}}, \set{\Gamma_2, \br[\tilde v, \tilde u]{\Query}\dbr{\Psi_z}\pairQ zC}[u_1, \ldots, u_n/b]
}{
	\infer[!]{
		\srv xaP \seq 
		\set[i]{\pairQ{u_i}{\query^\phl{x} B_i}}[\phl x/\phl a], \pairQ x{\bang^\phl{\tilde u} A} 
	}{
		\phl{P} \seq \set[i]{\pairQ{u_i}{\query^\phl{a} B_i}}, \br[\tilde u]{\Query}\pairQ aA
	}
	&
	\infer[?]{
		\client ybQ \seq 
		\set{\Gamma_2, \br[y]{\Query}\dbr{\Psi_z}\pairQ zC}[\phl y/\phl b], 
		\dbr{\Psi_2}\pairQ y{\query^\phl{z} \dual A}
	}{
		\phl{Q}\seq \Gamma_2, \dbr{\Psi_z}\pairQ zC, \dbr{\Psi_2}\pairQ b{\dual A}
	}
}
$$

\[
\left\{
\begin{array}{lcl}
	\set[i]{\pairQ{u_i}{\query^\phl{x} B_i}}[\phl x/\phl a]
	&\rhd &
	\pairQ x{\bang^\phl{\tilde u} A} 
	\\
	\set{\Gamma_2, \br[y]{\Query}\dbr{\Psi_z}\pairQ zC}[\phl y/\phl b]
	&\rhd &
	\dbr{\Psi_2}\pairQ y{\query^\phl{z} \dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\set[i]{\dbr{\Psi_{2u_i}}\pairQ{u_i}{\query^\phl{x} B'_i}}[\phl x/\phl a]
	&\rhd &
	\pairQ x{\bang^\phl{\tilde u} A} 
	\\
	\set{\Gamma'_2, \br[y]{\Query}\dbr{\Psi_z}\pairQ z{C'}}[\phl y/\phl b]
	&\rhd &
	\pairQ y{\query^\phl{z} \dual A}
\end{array}
\right\}
\]

\[
\longrightarrow_{\mathsf{subst}}
\left\{
\begin{array}{lcl}
	\set[i]{\dbr{\Psi_{2u_i}}\pairQ{u_i}{\query^\phl{z} B'_i}}[\phl x/\phl a]
	&\rhd &
	\pairQ x{A} 
	\\
	\set{\Gamma'_2, \br[\tilde u]{\Query}\dbr{\Psi_z}\pairQ z{C'}}[\phl y/\phl b]
	&\rhd &
	\pairQ y{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{subst}}
\Gamma
\]

$$
\quad\reducesto_\beta\quad
\infer[\tsc{Cut}]{
	\seq \Gamma
}{
	\phl{P} \seq 
	\set[i]{\pairQ{u_i}{\query^\phl{a} B_i}}, \br[\tilde u]{\Query}\pairQ aA
	&
	\phl{Q}\seq 
	\Gamma_2, \dbr{\Psi_z}\pairQ zC, \dbr{\Psi_2}\pairQ b{\dual A}
}
$$	
	
\[
\left\{
\begin{array}{lcl}
	\set[i]{\pairQ{u_i}{\query^\phl{a} B_i}}
	&\rhd &
	\br[\tilde u]{\Query}\pairQ aA
	\\
		\Gamma_2, \dbr{\Psi_z}\pairQ zC
	&\rhd &
	\dbr{\Psi_2}\pairQ b{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\set[i]{\dbr{\Psi_{2u_i}}\pairQ{u_i}{\query^\phl{a} B'_i}}
	&\rhd &
	\br[\tilde u]{\Query}\pairQ aA
	\\
	\Gamma'_2, \dbr{\Psi_z}\pairQ z{C'}
	&\rhd &
	\pairQ b{\dual A}
\end{array}
\right\}
\]
\[
\longrightarrow_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\set[i]{\dbr{\Psi_{2u_i}}\pairQ{u_i}{\query^\phl{z} B'_i}}
	&\rhd &
	\pairQ aA
	\\
	\Gamma'_2, \br[\tilde u]{\Query}\dbr{\Psi_z}\pairQ z{C'}
	&\rhd &
	\pairQ b{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{subst}}
\Gamma
\]



\mypar{Commutative $\tensor$ case}

\[
\infer[\cut]{
	\phl{\res {xy}(P\pp (\send z{v}{Q}{R}))}\seq 
	\Gamma 
}{
	\phl P\seq\Gamma_1, \set[j]{\dbr{\Psi_{w_j}}\pairQ{w_j}{E_j}}, \dbr{\Psi_1}\pairQ x{A}
	&
	\infer[\tensor]{
		\send z{v}{Q}{R}\seq 
		\Gamma_2,
		\{\br[z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\}_i,
		\br[z]{\Sigma}\dbr{\Psi_2}\pairQ y{\dual A},
		\dbr{\Psi_z}\pairQ z{B\tensor^{\phl{\tilde u y}} D}
	}{
		\phl {Q}\seq \{\Delta_i\}_i, \Sigma, \pairQ {v} {B}
		&
		\phl {R}\seq 
		\Gamma_2,
		\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\}_i,
		\dbr{\Psi_2}\pairQ y{\dual A}, \dbr{\Psi_z}\pairQ z{D}
	}
}
\]

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[j]{\dbr{\Psi_{w_j}}\pairQ{w_j}{E_j}}
	&\rhd &
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2,
	\{\br[z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\}_i, \dbr{\Psi_z}\pairQ z{B\tensor^{\phl{\tilde u y}} D}
	&\rhd& 
	\br[z]{\Sigma}\dbr{\Psi_2}\pairQ y{\dual A}
\end{array}
\right\}
\]
\[
\longrightarrow_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[j]{\br[z]{\Sigma_j}\bullet\dbr{\Psi_{w_j}}\pairQ{w_j}{E_j}}
	&\rhd &
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2,
	\{\bullet\br[z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\}_i, \bullet\dbr{\Psi_z}\pairQ z{B\tensor^{\phl{\tilde u \tilde w}} D}
	&\rhd& 
	\dbr{\Psi_2}\pairQ y{\dual A}
\end{array}
\right\}
\quad\text{with}\quad\Sigma = \set[j]{\Sigma_j}
\]
\[
\longrightarrow^*_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\Gamma'_1, \set[j]{\br[z]{\Sigma_j}\dbr{\Psi_{2w_j}}\dbr{\Psi_{w_j}}\pairQ{w_j}{E'_j}}
	&\rhd &
	\pairQ x{A}
	\\
	\Gamma'_2,
	\{\dbr{\Psi_{1u_i}}\br[z]{\Delta_i}\dbr{\Psi_{u_i}}\pairQ{u_i}{C'_i}\}_i, \dbr{\Psi_{1z}}\dbr{\Psi_z}\pairQ z{B\tensor^{\phl{\tilde u \tilde w}} D'}
	&\rhd& 
	\pairQ y{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{subst}}\Gamma
\]

We want to cut $\phl P$ and $\phl R$ together, as we can ultimately apply the induction hypothesis to this $\cut$ given that $\phl R$ is a subprocess of $\send z{v}{Q}{R}$:
\[
\infer[\cut]{
	\phl{\res{xy}(P \pp R)}
	\seq \Gamma_0
}{
	\phl P\seq\Gamma_1, \set[j]{\dbr{\Psi_{w_j}}\pairQ{w_j}{E_j}}, \dbr{\Psi_1}\pairQ x{A}
	&
	\phl {R}\seq 
	\Gamma_2,
	\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\}_i,
	\dbr{\Psi_2}\pairQ y{\dual A}, \dbr{\Psi_z}\pairQ z{D}
}\]


This gives us conclusion $\Gamma_0$ obtained by reproducing the $\longrightarrow^*_{\mathsf{distr}}$ rewriting sequence on $\dbr{\Psi_1}$ and $\dbr{\Psi_2}$ that we had above, followed by the deterministic $\longrightarrow^*_{\mathsf{subst}}$ sequence on $\pairQ{x}{A}$ and $\pairQ{y}{\dual A}$.

\[
\left\{
\begin{array}{lcl}
	\Gamma_1, \set[j]{\dbr{\Psi_{w_j}}\pairQ{w_j}{E_j}}
	&\rhd& 
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2,\{\dbr{\Psi_{u_i}}\pairQ{u_i}{C_i}\}_i, \dbr{\Psi_z}\pairQ z{D}
	&\rhd& 
	\dbr{\Psi_2}\pairQ y{\dual A}
\end{array}
\right\}
\]
\[
\longrightarrow^*_{\mathsf{distr}}
\left\{
\begin{array}{lcl}
	\Gamma'_1, \set[j]{\dbr{\Psi_{2w_j}}\dbr{\Psi_{w_j}}\pairQ{w_j}{E'_j}}
	&\rhd &
	\pairQ x{A}
	\\
	\Gamma'_2,
	\{\dbr{\Psi_{1u_i}}\dbr{\Psi_{u_i}}\pairQ{u_i}{C'_i}\}_i, \dbr{\Psi_{1z}}\dbr{\Psi_z}\pairQ z{D'}
	&\rhd& 
	\pairQ y{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{subst}}\Gamma_0
\]

Finally we can reconstruct the original conclusion $\Gamma$ by applying the $\tensor$ rule.

\[
\infer[\tensor]{
	\send zvQ{\res{xy}(P \pp R)}
	\seq \Gamma
}{
	\phl {Q}\seq \{\Delta_i\}_i, \Sigma, \pairQ {v} {B}
	&
	\phl{\res{xy}(P \pp R)}
	\seq \Gamma_0
}
\]

\mypar{Commutative $\parr$ case}

\[
\infer[\cut]{
	\phl {\res{xy} (P\pp \recv uvQ)}\seq \Gamma
}{
	\phl P\seq
	\Gamma_1, \dbr{\Psi_1}\pairQ x{A}
	&
	\infer[\parr]{
		\phl {\recv uvQ}\seq 
		\Gamma_2, \dbr{\Psi_u}\pairQ u{B\parr^{\phl z}C}, \dbr{\Psi_2}\pairQ{y} {\dual A}
	}{
		\phl {Q}\seq \Gamma_2, \dbr{\Psi_u}\br[z]{\pairQ v{B}}\pairQ u{C}, \dbr{\Psi_2}\pairQ{y} {\dual A}
	}
}
\]

\[
\left\{
\begin{array}{lcl}
	\Gamma_1
	&\rhd& 
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2, \dbr{\Psi_u}\pairQ u{B\parr^{\phl z}C}  
	&\rhd& 
	\dbr{\Psi_2}\pairQ{y} {\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma
\]

\[
\infer[\parr]{
	\recv uv{\res {xy}(P\pp Q)} \seq\Gamma
}{
	\infer[\cut]{
		\phl{\res {xy}(P\pp Q)} \seq \Gamma_0
	}{
		\phl P\seq
		\Gamma_1, \dbr{\Psi_1}\pairQ x{A}
		&
		\phl {Q}\seq \Gamma_2, \dbr{\Psi_u}\br[z]{\pairQ v{B}}\pairQ u{C}, \dbr{\Psi_2}\pairQ{y} {\dual A}
	}
}
\]

\[
\left\{
\begin{array}{lcl}
	\Gamma_1
	&\rhd& 
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2, \dbr{\Psi_u}\br[z]{\pairQ v{B}}\pairQ u{C}
	&\rhd& 
	\dbr{\Psi_2}\pairQ{y} {\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma_0
\]

\mypar{Commutative $\bot$ case}

\[
\infer[\cut]{
	\phl{\res{xy}(P \pp \wait zQ)}
	\seq
	\Gamma
}{
	\phl{P} \seq \Gamma_1, \dbr{\Psi_1}\pairQ{x}{A}
	&
	\infer[\bot]{
		\wait zQ \seq 
		\dbr{\Psi_2}\pairQ{y}{\dual A}, \Gamma_2,
		\dbr{\Psi_z}\pairQ{z}{\bot^\phl{v}},
		\dbr{\Psi_v}\pairQ{v}{C\ctx{\one^\phl{z\tilde{u}}}}
	}{
		\phl{Q} \seq
		\dbr{\Psi_2}\pairQ{y}{\dual A}, \Gamma_2,
		\dbr{\Psi_z}\br[v]{\Star}\pairQ{z}{\cdot}, \dbr{\Psi_v}\pairQ{v}{C\ctx{\one^\phl{z\tilde{u}}}}
	}
}
\]

\[
\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1
	&
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2,\dbr{\Psi_z}\pairQ{z}{\bot^\phl{v}},
	\dbr{\Psi_v}\pairQ{v}{C\ctx{\one^\phl{z\tilde{u}}}}
	&
	\dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}
\Gamma
\]


\[
\infer[\cut]{
	\phl{\res{xy}(P \pp Q)}
	\seq
	\Gamma_0
}{
	\phl{P} \seq \Gamma_1, \dbr{\Psi_1}\pairQ{x}{A}
	&
	\phl{Q} \seq
	\dbr{\Psi_2}\pairQ{y}{\dual A}, \Gamma_2,
	\dbr{\Psi_z}\br[v]{\Star}\pairQ{z}{\cdot}, \dbr{\Psi_v}\pairQ{v}{C\ctx{\one^\phl{z\tilde{u}}}}
}
\]

\[
\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1
	&
	\dbr{\Psi_1}\pairQ x{A}
	\\
	\Gamma_2,
	\dbr{\Psi_z}\br[v]{\Star}\pairQ{z}{\cdot}, \dbr{\Psi_v}\pairQ{v}{C\ctx{\one^\phl{z\tilde{u}}}}
	&
	\dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}
\Gamma
\]

\[
\infer[\bot]{
	\wait{z}{ \phl{\res{xy}(P \pp Q)}}
	\seq \Gamma
}{
	\phl{\res{xy}(P \pp Q)}
	\seq
	\Gamma_0
}
\]
	
\end{proof}










  
%%%%%%%%%% Marco's proof

%  By induction on the cut formula and the depth of the proof. Since
%  this rule is symmetric in its premise, we only consider permutations
%  on the right-hand side. 
%  \begin{itemize}
%  \item {\em Base Case} ($\tensor$ and $\parr$). Let $\phl x\not\in\Psi'_i$,
%    \begin{itemize}
%    \item $\mathcal D_1$: $\phl P\seq\{\Delta_i\}_i, \pairQ {z'} {A_1}$
%    \item $\mathcal D_2$: $\phl Q\seq\Gamma_1,
%      \{[\Psi'_i][\Psi''_i]\pairQ{z_i}{C_i}\}_i, [\Psi_1]\pairQ x{A_2}$
%    \item $\mathcal E$: $\phl R\seq\Gamma_2, [\Psi_2][^{\phl r}\pairQ w{\dual
%        A_1}]\pairQ y {\dual A_2}$
%    \item $\tensor\ \mathcal D_1\ \mathcal D_2$:
%      $\phl {\send x{z'}PQ} \seq\Gamma_1, \{[\Psi'_i][^{\phl
%        x}\Delta_i][\Psi''_i]\pairQ{z_i}{C_i}\}_i, [\Psi_1]\pairQ
%      x{A_1\tensor^{\phl {\tilde z}}A_2}$
%    \item $\parr\mathcal E$: 
%      $\phl{\recv ywR}\seq\Gamma_2, [\Psi_2]\pairQ y{\dual
%        A_1\parr^{\phl r}A_2}$
%    \item
%      $\cut\ (\tensor\ \mathcal D_1\ \mathcal D_2) (\parr\mathcal E)$:
%      $\Gamma$ such that
%      \[\left(
%          \begin{array}{ll}
%            \Gamma_1, \{[\Psi'_i][^{\phl
%            x}\Delta_i][\Psi''_i]\pairQ{z_i}{C_i}\}_i\rhd [\Psi_1]\pairQ
%            x{A_1\tensor^{\phl {\tilde z}}A_2}
%            \\
%            \Gamma_2 \rhd [\Psi_2]\pairQ y{\dual
%            A_1\parr^{\phl r}A_2}
%          \end{array}
%        \right)
%        \longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma\]
%    \end{itemize}
%
%	
%    We can then obtain:
%    \begin{itemize}
%    \item $\cuttwo\ \mathcal D_1\mathcal E$:
%      $\phl {\res{z'\rhd w}(P\pp R)}\seq\Gamma_2, [\Psi_2][^{\phl
%        r}\{\Delta_i\}_i]\pairQ y {\dual A_2}$
%    \item $\cut\ \mathcal D_2\ (\cuttwo\ \mathcal D_1\mathcal E)$:
%      $\Gamma'$ such that
%      \[
%        \left(
%          \begin{array}{l}
%            \Gamma_1,
%            \{[\Psi'_i][\Psi''_i]\pairQ{z_i}{C_i}\}_i\rhd [\Psi_1]\pairQ x{A_2}
%            \\
%            \Gamma_2\rhd [\Psi_2][^{\phl
%            r}\{\Delta_i\}_i]\pairQ y {\dual A_2}
%          \end{array}
%        \right) \longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma'
%      \]
%      By Lemma~\ref{lem:inv}, we have that for every $\Gamma$ we
%      can always find an identical $\Gamma'$ derivable above.
%    \end{itemize}
%
%
%
%  \item {\em Inductive Case} ($\tensor$, subcase 1).
%    \begin{itemize}
%    \item $\mathcal D$: $\phl P\seq\Gamma_1, [\Psi_1]\pairQ x{A}$
%    \item $\mathcal E_1$: $\phl {Q_1}\seq \{\Delta_i\}_i, \Delta, \pairQ {z'} {B_1}$ 
%    \item $\mathcal E_2$:
%      $\phl {Q_2}\seq \Gamma_2,
%      \{[\Psi'_i][\Psi''_i]\pairQ{z_i}{C_i}\}_i,\
%      [\Psi'][\Psi'']\pairQ y{\dual A}, \ [\Psi_2]\pairQ w{B_2}$
%    \item $\tensor\ \mathcal E_1\mathcal E_2$:\\
%      $\send w{z'}{Q_1}{Q_2}\seq \Gamma_2,
%      \{[\Psi'_i][\Delta_i][\Psi''_i]\pairQ{z_i}{C_i}\}_i,\
%      [\Psi'][\Delta][\Psi'']\pairQ y{\dual A},\ [\Psi_2]\pairQ
%      w{B_1\tensor^{\phl{\tilde z}} B_2}$
%    \item $\cut\ \mathcal D\ (\tensor\ \mathcal E_1\mathcal E_2)$:
%      $\phl{\res {xy}(P\pp (\send w{z'}{Q_1}{Q_2}))}\seq \Gamma $ such
%      that $\Gamma$ is obtained from
%      
%      Hence, we can construct:
%      \begin{itemize}
%      	\item $\cut\ \mathcal D\ \mathcal E_2$:
%      	$\phl{\res{xy}(P\pp Q_2)}\seq \Gamma'$ such that $\Gamma'$ is
%      	obtained from
%      
%\end{itemize}
%\end{itemize}
%
%  \item {\em Inductive Case} ($\tensor$, subcase 2). In this case, no
%    interference between $\tensor$ and $\cut$, trivial.
%
%
%
%  \item {\em Inductive Case} ($\parr$).
%    \begin{itemize}
%    \item $\mathcal D$: $\phl P\seq\Gamma_1, [\Psi_1]\pairQ x{A}$
%    \item $\mathcal E$:
%      $\phl {Q}\seq \Gamma_2', [\Psi][^z\pairQ w{B_1}]\pairQ r{B_2}, [\Psi_2]\pairQ
%      {y} {\dual A}$
%    \item $\parr\mathcal E$:
%      $\phl {\recv rwQ}\seq \Gamma_2', [\Psi]\pairQ r{B_1\parr^{\phl z}B_2}, [\Psi_2]\pairQ
%      {y} {\dual A}$
%    \item $\cut\ \mathcal D\ \parr\mathcal E$:
%      $\phl {\res(xy) (P\pp \recv rwQ)}\seq \Gamma$ such that $\Gamma$
%      is obtained from
%      
%      
%      Hence,
%      \begin{itemize}
%      \item $\cut\  \mathcal D\ \mathcal E$:
%        $\phl{\res xy(P\pp Q)}\seq \Gamma'$
%        such that $\Gamma'$ is obtained from
%        
%      Clearly, whatever $\Gamma'$ we obtain, we can always apply a
%      $\parr$ rule so that...
%      
%      
%        
%      \end{itemize}
%      
%    \end{itemize}
%    
%  \end{itemize}


==> extension.tex <==



This behaviour is captured by the notion of queues of \emph{boxed}
messages, i.e.~messages that are in-transit.
\[
\begin{array}{rcllllllll}
	\dbr \Psi & \coloncolonequals & \cdot 
	& \mid\quad \br[u]{\Star}
	& \mid\quad \br[u]{\pairQ yA}
	& \mid\quad \br[u]{\Query}
	& \mid\quad \br[u]{\Left}
	& \mid\quad \br[u]{\Right}
	& \mid\quad \dbr \Psi \dbr \Psi 
\end{array}
\]




Similarly, $\br[u]{\Star}$, $\br[u]{\Left}$ or $\br[u]{\Right}$, and
$\br[u]{\Query}$ indicate that a request for closing a session, a
branching request, or server invocation, respectively, has been
received and must be forwarded to either a single endpoint or a list
of endpoints.


We may use the abbreviation $\br[\tilde u]{\Symbol}$ for denoting the
$\br[u_1]{\Symbol}\ldots\br[u_n]{\Symbol}$ when
$\phl{\tilde u} = \phl{u_1}, \ldots, \phl{u_n}$.
%
In this case, we also assume the implicit rewriting
$\br[\emptyset]{\Symbol}\dbr{\Psi} \equiv \dbr{\Psi}$.
%
This notation is convenient as when needed we can refer to $\Psi$, the
set of all the elements that appear in $\dbr{\Psi}$ removing the
annotated brackets.

\begin{example}
	If
	$\dbr{\Psi} =
	\br[u]{\Left}\br[v]{\pairQ{x}{A}}\br[u]{\Query}\br[w]{\Left}$, then
	$\Psi = \set{\Left, \pairQ{x}{A}, \Query}$.
\end{example}


\begin{displaymath}
	\begin{array}{c}
		%		\infer[\tsc{Ax}]{
		%			\fwd xy\seq\pairQ{x}{\dual A}, \pairQ yA
		%		}{
		%			\text {match annotation in } A\text{ and } B
		%		}
		\infer[\tsc{Ax}]{
			\fwd xy\seq\pairQ{x}{\dual a}, \pairQ ya
		}{}
		%
		\qquad
		%
		\infer[\bot]{
			\wait xP \seq \Gamma, \dbr{\Psi}\pairQ{x}{\bot^u}
		}{
			\phl{P} \seq \Gamma, \dbr{\Psi}\br[u]{\Star}\pairQ{x}{\cdot}
		}
		%
		\qquad	
		%
		\infer[\one\ (\vec u \not= \emptyset)]{
			\close x \seq \set[i]{\br[x]{\Star}\pairQ{u_i}{\cdot}}, \pairQ{x}{\one^{\tilde u}}
		}{ }
		%
		\\\\
		%
		\infer[\parr]{
			\phl{\recv xyP} 
			\seq 
			\Gamma, \dbr{\Psi}\pairQ x{A \parr^{\phl u} B} % \phl b: B\{C^\perp \tensor^a\}
		}{
			\phl P 
			\seq 
			\Gamma, \dbr{\Psi}\br[u]{\pairQ yA}\pairQ xB
		}
		%
		\qquad
		%
		\infer[\tensor]{
			\phl{\send xy{P}Q} 
			\seq 
			\Gamma,
			\br[x]{\pairQ{z}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C},
			\dbr{\Psi_x}\pairQ x{A \tensor^u B}
		}{
			\phl {P}
			\seq
			\pairQ{z}{\dual {A(y)}},\pairQ y{A(z )}
			& 
			\phl Q 
			\seq
			\Gamma, \dbr{\Psi_u}\pairQ{u}{C}, \dbr{\Psi_x}\pairQ xB
		}
		%
		\\\\
		%
		\infer[\with]{
			\Case{x}{P}{Q}
			\seq \Gamma, \dbr{\Psi}\pairQ x{B \with^u C}
		}{
			\phl P\seq \Gamma, \dbr{\Psi}\br[u]{\Left}\pairQ xB
			&
			\phl Q\seq \Gamma, \dbr{\Psi}\br[u]{\Right}\pairQ xC
		}
		%
		\\\\
		%
		\infer[\oplus_l]{
			\inl xP\seq \Gamma, \br[x]{\Left}\dbr{\Psi_u} \phl u: \thl D,
			\dbr{\Psi_x}\pairQ x{B \oplus^u C}
		}{
			\phl P\seq \Gamma, \dbr{\Psi_u} \phl u: \thl C, \dbr{\Psi_x}\pairQ xB
		}
		%
		\qquad
		%
		\infer[\oplus_r]{
			\inr xP\seq \Gamma, \br[u]{\Right}\dbr{\Psi_u} \phl u: \thl D,
			\dbr{\Psi_x}\pairQ x{B \oplus^u C}
		}{
			\phl P\seq \Gamma, \dbr{\Psi_u} \phl u: \thl C, \dbr{\Psi_x}\pairQ xC
		}
		%
		\\\\
		%
		\infer[!\ (\vec u \not= \emptyset)]{
			\srv xyP \seq \set[i]{\pairQ{u_i}{\query^x B_i[x/y]}}, \pairQ x{\bang^{\tilde u} C} 
		}{
			\phl{P} \seq \set[i]{\pairQ{u_i}{\query^y B_i}}, \br[\tilde u]{\Query}\pairQ y C
		}
		%
		\qquad
		%
		\infer[?]{
			\client xyP \seq \set{\Gamma, \br[x]{\Query}\dbr{\Psi_z}\pairQ zC}[x/y], \dbr{\Psi_x}\pairQ x{\query^z C}
		}{
			\phl{P}\seq \Gamma, \dbr{\Psi_z}\pairQ zC, \dbr{\Psi_x}\pairQ yC
		}
		%
	\end{array}
\end{displaymath} 



Next, we consider three cases, depending on if the element is a queued message $\br[d]{\pairQ bB}$, a branch $\br[d]{\Left}$, or a session $\br[d]{\Query}$, and define the corresponding distribution rule parameterized by connectives $\mathbf{CO} \bnfas \tensor \bnfalt \oplus \bnfalt ?$, and
queues $\mathbf{Q} \bnfas {\pairQ bB} \bnfalt {\Left} \bnfalt {\Query}$. \carsten{Why is the $B$ not blue?}

$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\mathbf{CO}^\bhl{\bm x}}} & \rhd & \br[d]{\mathbf{Q}}\dbr{\Psi_1}\pairQ{x}{A}
	\\
	\Gamma_2, \dbr{\Psi_{1c}}\bullet\dbr{\Psi_c}\pairQ{c}{C}& \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
\xrightarrow{\br[d]{\mathbf{Q}}\circ \phl{c}}_{\mathsf{distr}}
$$

$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\mathbf{CO}^\bhl{\bm c}}} & \rhd & \dbr{\Psi_1}\pairQ{x}{A}\\
	\Gamma_2, \dbr{\Psi_{1c}}\br[d]{\mathbf{Q}}\bullet\dbr{\Psi_c}\pairQ{c}{C} & \rhd & \dbr{\Psi_2}\pairQ{y}{\dual A}
\end{array}
\right\}
$$
\noindent
where the  $\mathbf{CO}^x$ refers to the leftmost occurence of a $\mathbf{CO}$ labelled with $x$ in $D$.


We capture the substitution in one rule based on the top level collective $F = A (\mathbf{CO})^{\bhl{\bm b}} B$ and
its dual $F ^\perp = \dual A \mathbf{(\mathbf{CO}^\perp)}^{\bhl{\bm c}} \dual B$, which expresses that communication will commence between $x$ and $\bhl{\bm b}$, and $y$ and $\bhl{\bm c}$, respectively.  Note that we slightly abuse notation by writing $\mathbf{CO}^\perp$ for the dual connective of $\mathbf{CO}$.  Substitution progresses then in a rather straightforward way: Identify the type of channel $b$ ($x$) and the topmost element ($y$) in the queue for $c$ and then  record the newly established connection between $b$ and $c$ by replacing  $x$ by $c$ and $y$ by $b$.
The deceptive simple idea is capture by the following rule.

$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_b}\pairQ{b}{C\ctx{\mathbf{(\mathbf{CO}^\perp)}^\bhl{\bm x}}} & \rhd & \pairQ{x}{A (\mathbf{CO})^{\bhl{\bm b}} B} \\
	\Gamma_2, \br[\bhl{\bm y}] {\mathbf{Q}}\dbr{\Psi_c}\pairQ{c}{D} & \rhd &
	\pairQ{y}{\dual A \mathbf{(\mathbf{CO}^\perp)}^{\bhl{\bm c}} \dual B} \\
	\text{or } \Gamma_2, \dbr{\Psi'_c}\pairQ{c}{D\ctx{(\mathbf{CO})^\bhl{\bm y}}} && (y \not\in\dbr{\Psi'_c})
\end{array}
\right\}
\xrightarrow{\br[]{}\circ c}_{\mathsf{subst}}
$$
$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_b}\pairQ{b}{C\ctx{\mathbf{(\mathbf{CO}^\perp)}^\bhl{\bm c}}} & \rhd & \pairQ{x}{B} \\
	\Gamma_2, \br[\bhl{\bm b}]{\mathbf{Q}}\dbr{\Psi_c}\pairQ{c}{D} & \rhd &
	\phl y: \thl {B^\perp} \\
	\text{or } \Gamma_2,  \dbr{\Psi'_c}\pairQ{c}{D\ctx{(\mathbf{CO})^\bhl{\bm b}}}
\end{array}
\right\}
$$





%
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> gathering.tex <==
We can complexify the types in order to allow broadcasting and gathering.
\[
\begin{array}{rcllllllll}
	\thl{A,B} & \coloncolonequals & 
	\thl{a}
	\quad\mid\quad \thl{a^\perp} 
	\\ &
	\quad\mid\quad & \thl{\one^{[u_1, \ldots, u_n]}}&
	\quad\mid\quad &\thl{\bot^u} &
	\\ &
	\quad\mid\quad &\thl{(A\tensor^{[u_1,\ldots,u_n]} B)} &
	\quad\mid\quad & \thl{(A\parr^u B)} 
	\\ &
	\quad\mid\quad & \thl{(A\oplus^u B)} &
	\quad\mid\quad & \thl{(A\with^{[u_1, \ldots, u_n]} B)} 
	\\ &
	\quad\mid\quad & \thl{?^u A} &
	\quad\mid\quad & \thl{!^{[u_1, \ldots, u_n]} A} 
\end{array}
\]


Contexts need to be changed as well.
\[
\begin{array}{rcllllllll}
	\dbr \Psi & \coloncolonequals & \cdot 
	& \quad\mid\quad \br[u]{\Star}
	& \quad\mid\quad \br[u]{\pairQ yB}
	& \quad\mid\quad \dbr \Psi \dbr \Psi 
	\\ &&
	& \quad\mid\quad \br[u]{\Left}
	& \quad\mid\quad \br[u]{\Right}
	& \quad\mid\quad \br[u]{\Query}
\end{array}
\]
%

%$\br[u]{\Star}$, 
$\br[u]{\Left}$ (or $\br[u]{\Right}$) and
$\br[u]{\Query}$ indicate that %a request for closing a session, 
a branching request and  server invocation, respectively, has been
received and must be forwarded

When it needs to be forwarded to a list of endpoints,
we may use the abbreviation $\br[\tilde u]{\Symbol}$ for denoting the
$\br[u_1]{\Symbol}\ldots\br[u_n]{\Symbol}$ when
$\phl{\tilde u} = \phl{u_1}, \ldots, \phl{u_n}$.
%
In this case, we also assume the implicit rewriting
$\br[\emptyset]{\Symbol}\dbr{\Psi} \equiv \dbr{\Psi}$.
%





The rules then need to be adapted as follows.
\begin{displaymath}
	\begin{array}{c}
		\infer[\tsc{Ax}]{
			\fwd xy\seq\pairQ{x}{\dual a}, \pairQ ya
%			\fwd xy\seq\pairQ{x}{\dual A(\phl y)}, \pairQ y{A(\phl x)}
		}{}
		%
		\qquad
		%
		\infer[\bot]{
			\wait xP \seq \Gamma, \dbr{\Psi}\pairQ{x}{\bot^\phl{u}}
		}{
			\phl{P} \seq \Gamma, \dbr{\Psi}\br[u]{\Star}\pairQ{x}{\cdot}
		}
		%
		\qquad	
		%
		\infer[\one]{
			\close x \seq \set[i]{\br[x]{\Star}\pairQ{u_i}{\cdot}}, \pairQ{x}{\one^{\tilde u}}
		}{ }
		%
		\\\\
		%
		\infer[\parr]{
			\phl{\recv xyP} 
			\seq 
			\Gamma, \dbr{\Psi}\pairQ x{A \parr^\phl{u} B} % \phl b: B\{C^\perp \tensor^a\}
		}{
			\phl P 
			\seq 
			\Gamma, \dbr{\Psi}\br[u]{\pairQ yA}\pairQ xB
		}
		%
		\qquad
		%
		\infer[\tensor\ (\Delta_i \not= \emptyset)]{
			\phl{\send xy{P}Q} 
			\seq 
			\Gamma,
			\big\{\br[\phl x]{\Delta_i}\dbr{\Psi_i}\pairQ{u_i}{C_i}\big\}_i,
			\dbr{\Psi}\pairQ x{A \tensor^{\phl{\tilde u}} B}
		}{
			\phl {P}
			\seq
			\big\{\Delta_i\big\}_i,\pairQ yA
			& 
			\phl Q 
			\seq
			\Gamma, \big\{\dbr{\Psi_i}\pairQ{u_i}{C_i}\big\}_i,
			\dbr{\Psi}\pairQ xB
		}
		%
%		\infer[\tensor]{
%			\phl{\send xy{P}Q} 
%			\seq 
%			\Gamma,
%			\set[i]{\br[x]{\pairQ{z_i}{A_i}}\dbr{\Psi_i}\pairQ{u_i}{C_i}},
%			\dbr{\Psi}\pairQ x{A \tensor^{\tilde u} B}
%		}{
%			\phl {P}
%			\seq
%			\set[i]{\pairQ{z_i}{A_i}},\pairQ yA
%			& 
%			\phl Q 
%			\seq
%			\Gamma, \set[i]{\dbr{\Psi_i}\pairQ{u_i}{C_i}}, \dbr{\Psi}\pairQ xB
%		}
		%
		\\\\
		%
		\infer[\with\ (\tilde u \not= \emptyset)]{
			\Case{x}{P}{Q}
			\seq \Gamma, \dbr{\Psi}\pairQ x{A \with^\phl{\tilde u} B}
		}{
			\phl P\seq \Gamma, \dbr{\Psi}\br[\tilde u]{\Left}\pairQ xA
			&
			\phl Q\seq \Gamma, \dbr{\Psi}\br[\tilde u]{\Right}\pairQ xB
		}
		%
		\\\\
		%
		\infer[\oplus_l]{
			\inl xP\seq \Gamma, \br[x]{\Left}\dbr{\Psi_z} \phl z: \thl C,
			\dbr{\Psi_x}\pairQ x{A \oplus^\phl{z} B}
		}{
			\phl P\seq \Gamma, \dbr{\Psi_z} \phl z: \thl C, \dbr{\Psi_x}\pairQ xA
		}
%		\infer[\oplus_l]{
%			\inl xP\seq \Gamma, \br[\tilde u, x]{\Left}\dbr{\Psi_z} \phl z: \thl C,
%			\dbr{\Psi_x}\pairQ x{A \oplus^ z B}
%		}{
%			\phl P\seq \Gamma, \br[\tilde u]{\Left}\dbr{\Psi_z} \phl z: \thl C, \dbr{\Psi_x}\pairQ xA
%		}
		%
		\qquad
		%
		\infer[\oplus_r]{
			\inr xP\seq \Gamma, \br[x]{\Right}\dbr{\Psi_z} \phl z: \thl C,
			\dbr{\Psi_x}\pairQ x{A \oplus^\phl{z} B}
		}{
			\phl P\seq \Gamma, \dbr{\Psi_z} \phl z: \thl C, \dbr{\Psi_x}\pairQ xB
		}
%		\infer[\oplus_r]{
%			\inr xP\seq \Gamma, \br[\tilde u, x]{\Right}\dbr{\Psi_z} \phl z: \thl C,
%			\dbr{\Psi_x}\pairQ x{A \oplus^ z B}
%		}{
%			\phl P\seq \Gamma, \br[\tilde u]{\Right}\dbr{\Psi_z} \phl z: \thl C, \dbr{\Psi_x}\pairQ xB
%		}
		%
		\\\\
		%
		\infer[!\ (\tilde u \not= \emptyset)]{
			\srv xyP \seq \set[i]{\pairQ{u_i}{\query B_i}}, \pairQ x{\bang^\phl{\tilde u} A} 
		}{
			\phl{P} \seq \set[i]{\pairQ{u_i}{\query B_i}}, \br[\tilde u]{\Query}\pairQ y A
		}
		%
		\qquad
		%
		\infer[?]{
			\client xyP \seq \Gamma, \br[x]{\Query}\dbr{\Psi_z}\pairQ zC, \dbr{\Psi_x}\pairQ x{\query^\phl{z} A}
		}{
			\phl{P}\seq \Gamma, \dbr{\Psi_z}\pairQ zC, \dbr{\Psi_x}\pairQ yA
		}
%		\infer[?]{
%			\client xyP \seq \Gamma, \br[\tilde u, x]{\Query}\dbr{\Psi_z}\pairQ zC, \dbr{\Psi_x}\pairQ x{\query^\phl{z} A}
%		}{
%			\phl{P}\seq \Gamma, \br[\tilde u]{\Query}\dbr{\Psi_z}\pairQ zC, \dbr{\Psi_x}\pairQ yA
%		}
		%
	\end{array}
\end{displaymath} 

Proposition~\ref{prop:embed} is naturally extended to additives and exponentials.

\begin{proposition}\label{prop:embed2}
	Any forwarder is a CP-typable process, that is, if $\phl P \seq \Gamma$, then  $\phl P \cll \enc{\Gamma}$.
	%
	The embedding $\enc{\cdot}$ being extended as: $\enc{\br[u]{\Symbol}\dbr{\Psi}} = \enc{\dbr{\Psi}}$.
\end{proposition}





==> introduction-backup.tex <==
A concurrent system is more than a sum of processes. It also includes
the fabric that determines how processes are tied together.
% and through which information is exchanged.
%
Session types, originally proposed by Honda et al.~\cite{HVK98}, are
type annotations that ascribe protocols to processes in a concurrent
system and %, as a fabric,
determine how they behave when communicating
with each other. Such type annotations are useful for various
reasons. First, they serve as communication blueprints for the entire
system and give programmers clear guidance on how to implement
communication patterns at each endpoint (process or service).  Second,
they make implementations of concurrent systems safer, since
well-typedness entails basic safety properties of programs such as
{\em lack of communication errors} (``if the protocol says I should
receive, e.g., an integer, I will never receive, e.g., a boolean''),
{\em session fidelity} (``my programs follow the protocol
specification patterns''), and {\em in-session deadlock freedom}
(``the system never gets stuck by running a protocol'').
% Such basic properties are essential for programming safe communicating
% systems.
% Because of that, in recent years, session types have become a vibrant
% and active research area with  real-world world impact. 
% Session types are now actively integrated into mainstream programming
% languages such as Java~\cite{scribble}, Go~\cite{LNTY18},
% Erlang~\cite{F16}, and many more~\cite{ABCDimplementations}.
%
Intuitively, session types make sure that the processes are {\em compatible}
and that they exchange messages in the prescribed way for the
concurrent system to work correctly.
%
They do that by preventing messages from being duplicated, as
superfluous messages would not be accounted for, and by preventing
messages from getting lost, otherwise a process might get stuck,
awaiting a message.


In the case of \emph{binary sessions types}, type annotations of
protocols between two parties, % (binary protocols)
compatibility means for % session
type annotations to be dual to one another: the send action of one
party must be matched by a corresponding receive action of the other
party, % offered choices matched by selection,
and vice versa.  Curiously, binary session types find their logical
foundations in linear logic, as identified by Caires and
Pfenning~\cite{CP10,CP16} and later by Wadler~\cite{W12,W14}.  They
have shown that session types correspond to linear logic propositions,
processes to proofs, reductions in the operational semantics to cut
reductions in linear logic proofs, and compatibility to the logical
notion of duality for linear formulas.  Duality, thus, defines, for
the lack of a better word, the ``fabric'' through which two processes
communicate %in an idealised world,
while abstracting away from practical details, e.g., message delay,
message order, or message buffering.


The situation is not as direct for \emph{multiparty session
  types}~\cite{HYC08,HYC16}, % i.e., 
type annotations for protocols with more than two participants.
%
Carbone et al.~\cite{CMSY15,CLMSW16} extended Wadler's embedding of
binary session types into classical linear logic (CLL) to the
multiparty setting, by generalising duality to the notion of {\em
  coherence}.
%
They observed that the in-between fabric, through which multiple processes communicate, holds the very key to
understanding multiparty session types:
%
when forcing the type annotations to be {\em coherent}, one ensures
that sent messages will eventually be collected.
% , and choices eventually selected.
%
Coherence as a deductive system allows one to derive  % exactly these
compatible judgements, while proofs correspond precisely to multiparty
protocol specifications. % in the Curry-Howard style.
%
A key result is that coherence proofs can be encoded as well-typed (as
proofs in CLL) processes, called {\em arbiters}, which means that the
fabric can be modelled formally as a process-in-the-middle.
%
However, no precise logical characterisation of what constitutes
arbiters was given.
%
In this paper, we continue this line of research and define a
subsystem of processes, called \emph{asynchronous forwarders} or \emph{forwarders} in short, that
provides one possible such characterisation and also  guarantees multiparty session
compatibility.
%
%Synchronous forwarders allow us to model this fabric.


As the name already suggests, a forwarder is a process that forwards
messages, choices, and services from one endpoint to another according
to the protocol specification.
% given as a multiparty session type.
% It should not be confused with the simple forwarder processes that are
% typed by the axiom rule in~\cite{CP16,W14}.
Intuitively, similarly to an arbiter, a forwarder process mimics the
fabric by capturing the message flow.  However, when data-dependencies
allow, forwarders could, in theory, non-deterministically choose to
receive messages from different endpoints, and then forward such
messages at a later point. Or, they can also decide to buffer a
certain number of messages from a given receiver.  Eventually,
% synchronous forwarders are a class of forwarders that
they
%
re-transmit messages only after receiving them,
% using a one-size buffer,
without interpreting, modifying, or computing with them.
%

In this work, asynchronous forwarders support buffers of unlimited
size.
% 1 -- only one message can be stored for each endpoint at a given
% time.
This  preserves the order of messages from the same sender, i.e., after
receiving a message from one party, the forwarder enqueues it until the message is delivered to its
destination.
% Forwarders
% supporting larger buffer sizes are not discussed here, but left to
% future work.
%
Forwarders can be used to explain communication patterns as they
occur in practice, such as message routing, proxy services, and
runtime monitors for message flows~\cite{JGP16}.
%
% We leave this investigation to future work.  

%\todo{rephrase this paragraph for asynchronous forwarders!}
The meta-theoretic study of forwarders allows us to
conclude that there is a correspondence between forwarders and multiparty compatibility.
%
Forwarders are stronger than coherence and can be used to guide the communication of multiple processes similarly to the multi-cut elimination in~\cite{CLMSW16} and so they are a way to justify multiparty compatibility.
%
The reverse direction also holds, i.e., if a multiparty session of processes is compatible, they can be linked by a forwarder; in such a way, forwarders as a logic provide a proof theory for multiparty compatibility.
%
In this paper, we also show that 
forwarders can safely be composed through cut elimination, which
allows us to combine the fabric between two concurrent systems
(figuring arbitrary many processes). 
%
%With respect to multiparty compatibility, we
%prove their {\em soundness}, namely that any multiparty compatibility proof can be
%emulated by a forwarder simulating the actions of the
%fabric, and their {\em completeness}, meaning that every 
%forwarder guarantees correct multiparty communication. 

\smallskip

\mypar{Outline and key contributions.}  The key contributions of this
paper include
\begin{itemize}
\item a logical characterisation of \emph{forwarders}
  (\S~\ref{sec:forwarders});
\item a reductive operational semantics based on cut-elimination
  (\S~\ref{sec:semantics});
\item a correspondence between multiparty compatibility and %asynchronous
forwarders, generalising coherence: every 
forwarder guarantees correct multiparty communication (\S~\ref{sec:mcut}) 
and any compatible multiparty session can be
emulated by a forwarder (\S~\ref{sec:mcompatibility}).
\end{itemize}
Additionally, \S~\ref{sec:preview} gently introduces the main concepts
on an example and \S~\ref{sec:prelim} recaps the definitions of types,
processes, and CP-typing, while \S~\ref{sec:related} discusses related
and future work and concluding remarks are in
\S~\ref{sec:conclusions}.



%(NEW) Contributions:
%\begin{itemize}
%\item logical characterisation of forwarders
%\item correspondence between multiparty compatibility and asynchronous
%  forwarders, generalising coherence.
%\item reductive operational semantics based on cut-elimination
%\end{itemize}

% In Section~\ref{sec:sync_system}, we introduce synchronous
% forwarders as a proof system.  In Section~\ref{sec:cut-elim}, we
% prove the cut-elimation result for synchronous forwarders, ensuring
% their compositionality.  In Section~\ref{sec:coherencesf} we
% demonstrate the tight correspondence of synchronous forwarders and
% coherence, i.e., we show that a forwarder is {\em synchronous} if
% and only if it is {\em coherent}.
% Finally, we conclude this paper with some discussions of
% related and future work.

% Through an algorithm that allows to permute actions of a
% process, we can always reconstruct an arbiter, which can then be
% mapped back to a coherence proof. The advantage of using synchronous
% forwarders rather than just arbiters is the former allow for different
% behaviour to happen. As a consequence, arbiters are just special
% instances of forwarders.

%  In this work, with a Curry-Howard
% approach, we identify a class of forwarders, dubbed {\em synchronous
%   forwarders}, by defining a proof system equipped with cut
% elimination which is a restriction of CLL. Synchronous forwarders are
% a class of session-typed forwarding processes that forward messages
% between endpoints. That is done synchronously, i.e., they can buffer
% at most one message at the time from each sender.

% As a
% consequence, it shows that systems with multiparty session types can
% be simulated by systems with only binary session types.
%  This is the same notion of coherence which we will characterize using synchronous forwarders. 

% identified a correspondence between
% {\em binary session types}, a version of session types that deals only
% with protocols between two parties (binary protocols), and
% intuitionistic linear logic Two years later,
%  proposed a similar correspondence between
% session types and classical linear logic (CLL).
% More recently, Carbone
% et al.~\cite{CMYS15,CLMSW16} extended the work of Wadler to work with
% a generalisation of binary session types, known as {\em multiparty
%   session types}~\cite{HYC08,HYC16}, by defining a proof system called
% {\em coherence} whose proofs correspond to multiparty protocol
% specifications in the Curry-Howard style. A key contribution of their
% work shows that coherence proofs can actually be encoded as well-typed
% processes, called {\em arbiters}, corresponding to proofs in CLL. As a
% consequence, it shows that systems with multiparty session types can
% be simulated by systems with only binary session types.

% One particular feature of arbiters is that they act as glue in the
% system, by forwarding messages from one endpoint to another according
% to the protocol specification given as a multiparty session type. The
% intuition behind is that whenever we wish to enforce a communication
% protocol between the endpoints of a concurrent system, we can always
% implement it by adding a middle forwarding process which enforces
% where messages should flow. Often such processes are referred to as
% {\em forwarders}, processes that retransmits previously received
% messages, without interpreting, modifying, or computing with them.
% Forwarders can be used to model the exchange of messages between peers
% in a {\em multiparty} computation. They can also be used to explain
% communication patterns as they occur in practice, such as message
% routing, proxy services, and runtime monitors for message flows.
% %
% Contrary to popular belief, forwarders are not just simple processes,
% but they satisfy some basic principles that differentiate them from
% standard processes. 

%
% Synchronous forwarders can be safely composed (cut elimination). But
% more importantly, synchronous forwarders are a generalisation of
% arbiters. Through an algorithm that allows to permute actions of a
% process, we can always reconstruct an arbiter, which can then be
% mapped back to a coherence proof. The advantage of using synchronous
% forwarders rather than just arbiters is the former allow for different
% behaviour to happen. As a consequence, arbiters are just special
% instances of forwarders.

% In a multiparty setting, we wish to compose several processes at once,
% with the goal of having safe communications among the various
% processes. However, in this case, things get more
% complicated. Consider for example the case in which we wish to compose
% three processes $P$, $Q$, and $R$ with endpoints $x$, $y$, and $z$
% respectively, such that $x$ had type $A$, $y$ has type $B$ and $z$ has
% type $C$. In such case, we can have one-to-one communications between
% any two endpoints and compatibility has to make sure that nothing goes
% wrong. For example, $x: A_1\tensor A_2\parr \perp$,
% $y: A_1^\perp\parr \one$, and $z: A_2^\perp\tensor\one$ are compatible
% ($x$ can send a message to $y$ and then $z$ can send a message to $x$
% reaching the safe state in which $x:\perp$, $y:\one$ and
% $z:\one$). However, $x: A_1\tensor A_2\tensor \perp$,
% $y: A_1^\perp\parr \one$, and $z: A_2^\perp\tensor\one$ are not
% compatible because they would reach a deadlock in which $x$ wishes to
% send something of type $A_2$, $z$ something of type $A_2^\perp$, while
% $y$ would be done. Carbone et al.~\cite{CMSY15,CLMSW16} show that such
% a concept of {\em multiparty compatibility} can be captured by an
% proof system called {\em coherence} whose proof terms are nothing by
% the global types know from multiparty session types. [DESCRIBE HERE
% THE PECULARITY OF COHERENCE $==>$ SWAPPING]

% A further interesting result~\cite{CLMSW16} shows that coherence
% proofs can be translated into actual processes (dubbed {\em arbiters}
% by the authors) which work as coordinator processes that receive and
% resend messages between the compatible proceses, simulating how the
% processes composed with coherence should exchange messages.

% Such arbiters have a very key behaviour: they act as those well-known
% processes that can be found in concurrent systems, often referred to
% as {\em forwarders}. [SAY WHAT FORWARDERS ARE, MAYBE RECYCLE FROM
% DEFINITION OF POPL SUBMISSION]

% If we look at the image of the translation of coherence into
% processes, we can spot a few key features about them: i) they are
% forwarders; ii) they have a very simple structure, i.e., for each
% forwarding operation, they first input all the necessary information
% from some endpoints, and then they forward such information on to
% other endpoints. [EXAMPLE HERE] However, if we refer to the notion of
% forwarder a forwarder can also have alternative behaviour. I.e., it
% could actually receive all possible messages first also concerning
% separate forwarding operations and then decide to forward at a later
% time. For example, [HERE PICK THE EXAMPLE ABOVE and EXPAND].

% Based on the observation above, we can see that there is a bigger
% class of forwarders that is somehow equivalent to the mapping of
% coherence into processes. Hence, we ask: {\em can we define a proof
%   system that characterises those processes that are equivalent to the
%   image of coherence as a proof system that is a restriction of linear
%   logic?}. Answering positively to this question would allow us to
% precisely describe such systems and ??? WHY IS THAT INTERESTING ??????

% Coherence for multiparty session types is a notion
% that defines compatibility of processes via a given
% protocol. \cite{CLMSW16} show that coherence is also a
% program-as-proofs representation of such protocols (known as global
% types). As a corollary from our results we freely obtain a procedure
% for composing coherence proofs (hence also global types) 
% to support proof compositionality. (\S~\ref{sec:coherence})

%  One can think of a global type as the glue between endpoints,
%  computationally limited but operationally adequately
%  powerful

%  Global types can be translated into processes, and as such can be put into 
% (Curry-Howard) correspondence to a proof in linear logic (identified originally for intuitionistic linear logic
% by ~\cite{CPT16} and later for classical linear logic
% by~\cite{W14}). 
% However, not every proof in linear logic corresponds to
% a global type so we identify precisely the fragment of linear logic that carves out coherence proofs.


%  Our ultimate goal is to understand more genrally processes that
%  forwards messages in a multiparty setting, among several processes, which has
%  not been given a proncipled treatment before.
 
%  In this work, inspired by the Curry-Howard correspondence
%  between linear logic and the session-based
%  $\pi$-calculus~\cite{CPT16,W14}, we explore a subsystem of linear
%  logic that is the exact pendant to coherence.
 
% We draw inspiration from~\cite{JGP16,GJP18} that have recently proposed a system
%  that models {\em identity providers}, basically forwarders between
%  two channels.
%  %
%  Indeed, in  concurrency theory, the notion of forwarder has been formalised in
%  different contexts, for example, in the behavioural theory of the
%  $\pi$-calculus, \cite{S96} introduces a notion of forwarder for the
%  internal $\pi$-calculus, where a forwarder is defined as a process
%  that forwards all messages between {\em two} channels. More recently,
%  forwarders were instrumental in the work of~\cite{CPT16,W14}, where
%  their semantics corresponds to that of 
%  the linear logic axiom $\vdash A,A^\perp$.


% \paragraph{Our Contributions.}

% \paragraph{A running  example.}
% As a running example throughout this paper we use the classic
% \emph{2-buyer protocol}~\cite{HYC16}. Two buyers, $\phl{B_1}$ and
% $\phl{B_2}$, attempt to buy a book together from a seller $\phl
% S$. First, $\phl{B_1}$ sends the title of the book that she wishes to
% purchase to $\phl S$, who in turn sends a quote to both $\phl {B_1}$
% and $\phl {B_2}$. Then, $\phl{B_1}$ decides on how much she wishes to
% contribute and informs $\phl{B_2}$, who either pays the rest or
% cancels the transaction.

% In this example, a forwarder process (also called arbiter 
% in~\cite{CLMSW16}), say $\phl {P_1}$, can relay messages between
% $\phl{B_1}$, $\phl{B_2}$ and $\phl S$, enforcing the 2-buyer
% protocol. More precisely, the forwarder first receives the title from
% $\phl{B_1}$ and then forwards it to $\phl S$. It then receives the
% quote from $\phl S$ and forwards it to $\phl {B_1}$ and
% $\phl{B_2}$. Next, it collects an amount from $\phl{B_1}$ and forwards
% it to $\phl{B_2}$, and finally it relays the decision of $\phl{B_2}$
% to buy or not to buy to $\phl S$.

% This example can be extended by a second forwarder $\phl{P_2}$: assume
% that $\phl{B_2}$ wishes to delegate the decision to buy or not to buy
% to two colleagues, $\phl{C_1}$ and $\phl{C_2}$. Only if $\phl{C_1}$
% and $\phl{C_2}$ agree, the book will be bought.  The forwarder
% orchestrating the communication between $\phl{C_1}$, $\phl{C_2}$ and
% $\phl{B_2}$ does the following: it forwards the price to $\phl{C_1}$,
% and $\phl{B_1}$'s contribution to $\phl{C_2}$.  Then it relays
% decisions from $\phl{C_1}$ to $\phl{B_2}$ and from $\phl{C_2}$ to
% $\phl{B_2}$.
% %
% Intuitively, we should be able to combine $\phl {P_1}$ and
% $\phl {P_2}$ into a new forwarder $\phl P$ that orchestrates the
% communication between $\phl S$, $\phl{B_1}$, $\phl{B_2}$, $\phl{C_1}$
% and $\phl{C_2}$.  
%  \todo{do you perhaps have a drawing of the 2-buyers protocol somewhere
%    or should we attempt to make a new one maybe? }



%
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> semantics-bits.tex <==
\sonia{I propose to get rid of $\cuttwo$ and streamline the proof using the lemma below}

\carsten{what is rank and size in Lemma 5, and what do we need that for?}

\begin{lemma} %[Admissibility of  \cuttwo]
	\label{lem:cuttwo-adm}
  Let $\phl P\seq\pairQ z{\dual A}, \pairQ xA$ and
  $\phl Q\seq\Gamma, \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ y{B}$.
  Then, there exists $\phl R$ such that
  $\phl R\seq^\cut \Gamma, \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ y{B}$
  and $\mathtt{rank}(\phl{R}) = \mathtt{size}(A)$.
  %
  We denote this process as $\phl R = \phl{\res{x\rhd w}(P\pp Q)}$
\end{lemma}

\begin{proof}
	By induction on the structure of $\phl Q$.
	
	Because of the shape of its typing environment, $\phl Q$ cannot be of the shape $\fwd ab$ nor of the shape $\close a$.
	
	Case $\phl Q = \send uvST$ and $\phl w\in \mathtt{fn}(\phl S)$.
	%
	Assume we have the following
	\[
	\infer[\tensor]{
		\phl{\send uvST} 
		\seq 
		\Gamma', \br[u]{\pairQ w{\dual A}}\dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ u{A \tensor^y C}
	}{
		\phl{S} \seq \pairQ w{\dual A}, \pairQ vA
		&
		\phl{T} \seq
		\Gamma', \dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ uC
	}
	\]
%	where $\Gamma = \Gamma', \dbr{\Psi_u}\pairQ u{A \tensor^y C}$ and $\br[u]{...}\not\in\dbr{\Psi_1}$ -- so we can permeate $\br[u]{\pairQ{z}{\dual A}}$ to the top and we write $\dbr{\Psi_y}$ for $\dbr{\Psi_1}\dbr{\Psi_2}$.
%
We can take $\phl R = \send uv{\res{xw}(P\pp S)}T$ and indeed $\mathtt{rank}(\phl R) = \mathtt{size}(A)$ as follows:
%	
	\[
	\infer[\tensor]{
		\send uv{\res{xw}(P\pp S)}T
		\seq
		\Gamma', \br[u]{\pairQ z{\dual A}}\dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ u{A \tensor^y C}
		}{	
		\infer[\cut]{
			\phl{\res{xw}(P\pp S)} \seq \pairQ z{\dual A}, \pairQ vA
			}{
			\phl{P} \seq \pairQ z{\dual A}, \pairQ xA
			&
			\phl{S} \seq \pairQ w{\dual A}, \pairQ vA
		}
		&
		\phl{T} \seq
		\Gamma', \dbr{\Psi_y}\pairQ yB, \dbr{\Psi_u}\pairQ uC
		}
	\]
	
	\sonia{This could be simplified to $\phl{\send ux{P}T}$ in this context and would not need a $\cut$ but not in the general case cf.~appendix.} 
	
	Case $\phl Q = \send uvST$ and $\phl w\in \mathtt{fn}(\phl T)$.
	%
	Assume we are in the following context %$\Gamma = \Gamma', \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}$.
	\[
	\infer[\tensor]{
		\send uvST
		\seq
		\Gamma', \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}
	}{
		\phl{S} \seq \pairQ f{\dual F}, \pairQ vF
		&
		\phl T
		\seq
		\Gamma', \dbr{\Psi_1}\br[u]{\pairQ w{\dual A}}\dbr{\Psi_2}\pairQ yB, \dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{C}
	}
	\]
%	
	By applying the induction hypothesis to $\phl P$ and $\phl T$ (which indeed is a subprocess of $\phl Q$), we obtain $\phl{R_0}$ such that
	$\phl{R_0}\seq^\cut \Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{C}$
	and  $\mathtt{rank}(\phl{R_0}) = \mathtt{size}(A)$.
	%
	So we can take $\phl R = \send uvS{R_0}$
%
%	\[
%	\infer[\tensor]{
%		\send uvS{R_0}
%		\seq^\cut
%		\Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}
%	}{
%		\phl{S} \seq \pairQ f{\dual F}, \pairQ vF
%		&
%			\phl{R_0}
%			\seq^\cut
%			\Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{C}
%	}
%	\]
%	
	and indeed, $\phl R \seq^\cut \Gamma', \dbr{\Psi_1}\br[u]{\pairQ z{\dual A}}\dbr{\Psi_2}\pairQ yB, \br[u]{\pairQ f{\dual F}}\dbr{\Psi_d}\pairQ dD, \dbr{\Psi_u}\pairQ u{F \tensor^d C}$ and $\mathtt{rank}(R) = \mathtt{size}(A)$.
	
	When $\phl Q$ is of any other shape we can apply the induction hypothesis in a similar (or even simpler) way. 
      \end{proof}

      \begin{theorem} [Admissibility of Cut]
  Let $\phl P\seq\Gamma_1, [\Psi_1]\pairQ xA$ and
  $\phl Q\seq\Gamma_2, [\Psi_2]\pairQ y{A^\perp}$.  
  Then, for
  any $\Gamma$ such that
  $\big(\Gamma_1\rhd[\Psi_1]\pairQ xA,\ \Gamma_2\rhd[\Psi_2]\pairQ y{\dual
    A}\big)\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma$
  there exists $\phl R \seq \Gamma$.
\end{theorem}

\begin{proof}
	
	We proceed by lexicographic induction on  the pair of the size of $A$ and the sum of the size of $\phl P$ and $\phl Q$.
	That is, the induction hypothesis may be applied whenever 
	($i$) the rank of the cut is smaller,
%	 or ($ii$) the rank stays the same and a $\cuttwo$ is replaced by a $\cut$, 
	or ($ii$) the rank stays the same and one of the heights of derivations above the cut is smaller and the other is smaller or stays the same.
	
	\todo{Commutative case and axiom case.}
	
	\mypar{Units} 
	$$
	\infer[\textsc{Cut}]{
		\phl{\res {xy}(\close x \pp \wait {y}{P}  )} \seq 
		\Gamma
	}{
		\infer[\one]{
			\close x \seq 
			\set[i]{\br[x]{\Star}\pairQ{u_i}{\cdot}}, \pairQ{x}{\one^\phl{\tilde u}}
		}{}
	&
	\infer[\bot]{
		\wait yP \seq 
		\dbr{\Psi}\pairQ{y}{\bot^\phl{v}}, \Gamma_2,\dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}}
	}{
		\phl{P} \seq
		 \dbr{\Psi}\br[v]{\Star}\pairQ{y}{\cdot}, \Gamma_2,\dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}}
	}
	}
	$$
	$$
	\quad\reducesto_\beta\quad
	\infer[y \leadsto \tilde u]{
		\phl{P^\mathsf{y \leadsto \tilde u}}
		\seq
		\set[i]{\dbr{\Psi_i}\br[v]{\Star}\pairQ{u_i}{\cdot}},
		\Gamma_2^\mathsf{y \leadsto \tilde u},\dbr{\Psi_c}\pairQ{v}{C^\mathsf{y \leadsto \tilde u}\ctx{\one^\phl{\tilde{z_1}{\tilde u}\tilde{z_2}}}}
		}{
		\phl{P} \seq \dbr{\Psi}\br[v]{\Star}\pairQ{y}{\cdot}, \Gamma_2, \dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}}
		}
	$$
	
	\sonia{This is a special rule. It is NOT a uniform substitution replacing $\phl y$ by $\phl {\tilde{u}}$ but it reproduces the changes performed by the distribution of $\Psi$ over the $\phl{u_i}$s.}
	

	
	$$
	\left\{
	\begin{array}{rcl}
		\set[i]{\br[x]{\Star}\pairQ{u_i}{\cdot}} & \rhd & \pairQ{x}{\one^{\tilde u}}\\
		\Gamma_2,\dbr{\Psi_c}\pairQ{v}{C\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}} & \rhd & \dbr{\Psi}\pairQ{y}{\bot^v}
	\end{array}
	\right\}
%	$$
%	$$
	\xrightarrow{}_{\mathsf{distr}}^*
	\left\{
	\begin{array}{rcl}
		\set[i]{\dbr{\Psi_i}\br[x]{\Star}\pairQ{u_i}{\cdot}} & \rhd & \pairQ{x}{\one^{\tilde u}}\\
		\Gamma_2^\mathsf{y \leadsto \tilde u},\dbr{\Psi_c}\pairQ{v}{C^\mathsf{y \leadsto \tilde u}\ctx{\one^\phl{\tilde{z_1}{y}\tilde{z_2}}}} & \rhd & \pairQ{y}{\bot^v}
	\end{array}
	\right\}
	$$
	$$
	\xrightarrow{}_{\mathsf{subst}}
	\set[i]{\dbr{\Psi_i}\br[v]{\Star}\pairQ{u_i}{\cdot}},
	\Gamma_2^\mathsf{y \leadsto \tilde u},\dbr{\Psi_c}\pairQ{v}{C^\mathsf{y \leadsto \tilde u}\ctx{\one^\phl{\tilde{z_1}{\tilde u}\tilde{z_2}}}}
	= \Gamma
	$$  
	
	
%	Knowing that the first step of the series of distribution looks like this:
%	$$
%	\left\{
%	\begin{array}{rcl}
%		\set[i\setminus k]{\bullet\br[x]{\Star}\pairQ{u_i}{\cdot}} , \bullet\br[x]{\Star}\pairQ{u_k}{\cdot}& \rhd & \pairQ{x}{\one^{\tilde u}}\\
%		\Gamma_2', \dbr{\Psi_d}\pairQ{d}{D\ctx{\tensor^\phl{y}}}& \rhd & \br[d]{\pairQ{b}{B}}\dbr{\Psi'}\pairQ{y}{\bot^v}
%	\end{array}
%	\right\}
%	\xrightarrow{}_{\mathsf{distr}} %\br[d]{\pairQ bB}\circ \phl{u_k}
%	\left\{
%	\begin{array}{rcl}
%		\set[i]{\bullet\br[x]{\Star}\pairQ{u_i}{\cdot}}, \br[d]{\pairQ{b}{B}}\bullet\br[x]{\Star}\pairQ{u_k}{\cdot} & \rhd & \pairQ{x}{\one^{\tilde u}}\\
%		\Gamma_2', \dbr{\Psi_d}\pairQ{d}{D\ctx{\tensor^\phl{u_k}}}& \rhd & \dbr{\Psi'}\pairQ{y}{\bot^v}
%	\end{array}
%	\right\}
%	$$
%	
	
	
	
	
	\mypar{Multiplicatives}
	$$
	\infer[\textsc{Cut}]{
		\phl{\res{xy}(\send xa{P}{Q} \pp \recv yc{R}) }
		\seq
		\Gamma
	}{
		\infer[\tensor]{
			\phl{\send xa{P}{Q}} 
			\seq 
			\Gamma_1,
			\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C},
			\dbr{\Psi_1}\pairQ x{A \tensor^u B}
		}{
			\phl {P}
			\seq
			\pairQ{d}{\dual A},\pairQ aA
			& 
			\phl {Q} 
			\seq
			\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C}, \dbr{\Psi_1}\pairQ xB
		}
		&
		\infer[\parr]{
			\phl{\recv yc{R}} 
			\seq 
			\dbr{\Psi_2}\pairQ y{\dual A \parr^v \dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}
		}{
			\phl {R}
			\seq 
			\dbr{\Psi_2}\br[v]{\pairQ c{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}
		}
	}
	$$
	
	$$
	\quad\reducesto_\beta\quad
	\infer[\tsc{Cut}]{
		\phl {\res{xy} (Q\pp \res{a\rhd c} (P\pp R))}
		\seq
		\Gamma
	}{
		\phl {Q} 
		\seq
		\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C}, \dbr{\Psi_1}\pairQ xB
		&
%		\infer[\tsc{Cut$_2$}]{
			\phl {\res{a\rhd c} (P\pp R)}
			\seq 
			\dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}
%		}{
%			\phl {P}
%			\seq
%			\pairQ{d}{\dual A},\pairQ aA
%			&
%			\phl {R}
%			\seq 
%			\Gamma_2, \dbr{\Psi_2}\br[v]{\pairQ c{\dual A}}\pairQ y{\dual B}
%		}
	}
	$$

By Lemma~\ref{lem:cuttwo-adm}, we know that $\phl S = \phl{\res{a\rhd c}(P\pp R)}$ exists, that $\phl S \seq^\cut \dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}$, and that its rank is equal to the size of $A$. 
%
By induction hypothesis any cut in the derivation of $\phl S$ are admissible as $\mathtt{rank}(\phl S) = \mathtt{size}(A) < \mathtt{size}(A \tensor^u B)$, that means in fact that $\phl S \seq \dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}, \Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}}$ without cut, which gives us the right premiss above.
%
Then, the new $\cut$ (on $B$) is also admissible by induction hypothesis on the rank as $\mathtt{size}(B) < \mathtt{size}(A \tensor^u B)$.

$$
\left\{
\begin{array}{rcl}
	\Gamma_1,
	\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C} & \rhd & 
	\dbr{\Psi_1}\pairQ x{A \tensor^u B}\\
	\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}} & \rhd &  \dbr{\Psi_2}\pairQ y{\dual A \parr^v \dual B} 
\end{array}
\right\}
%\xrightarrow{}_{\mathsf{distr}}^*
%$$
%
%$$
%\left\{
%\begin{array}{rcl}
%	\Gamma_1',
%	\dbr{\Psi_{2e}}\bullet\dbr{\Psi_e}\pairQ{e}{E\ctx{\tensor^\phl{ x}}} & \rhd & 
%	\br[e]{\pairQ fF}\dbr{\Psi_1'}\pairQ x{A \tensor^u B}\\
%	\Gamma_2', \dbr{\Psi_{1g}}\bullet\dbr{\Psi_g}\pairQ{g}{G} & \rhd &  \dbr{\Psi_2'}\pairQ y{\dual A \parr^v \dual B} 
%\end{array}
%\right\}
%$$
%$$
%\xrightarrow{\br[e]{\pairQ fF}\circ \phl{g}}_{\mathsf{distr}}
%\left\{
%\begin{array}{rcl}
%	\Gamma_1',
%	\dbr{\Psi_{2e}}\bullet\dbr{\Psi_e}\pairQ{e}{E\ctx{\tensor^\phl{g}}} & \rhd & 
%	\dbr{\Psi_1'}\pairQ x{A \tensor^u B}\\
%	\Gamma_2', \dbr{\Psi_{1g}}\br[e]{\pairQ fF}\bullet\dbr{\Psi_g}\pairQ{g}{G} & \rhd &  \dbr{\Psi_2'}\pairQ y{\dual A \parr^v \dual B} 
%\end{array}
%\right\}
%$$
%
%$$
\xrightarrow{}_{\mathsf{distr}}^*
\left\{
\begin{array}{rcl}
	\Gamma_1'',
	\dbr{\Psi_{2u}}\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
	\pairQ x{A \tensor^u B}\\
	\Gamma_2'', \dbr{\Psi_{1v}}\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{y}}} & \rhd &  \pairQ y{\dual A \parr^v \dual B} 
\end{array}
\right\}
$$

$$
\xrightarrow{}_{\mathsf{subst}}
\left\{
\begin{array}{rcl}
	\Gamma_1'',
	\dbr{\Psi_{2u}}\br[v]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
	\pairQ x{B}\\
	\Gamma_2'', \dbr{\Psi_{1v}}\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{u}}} & \rhd &  \pairQ y{\dual B} 
\end{array}
\right\}
\xrightarrow{}_{\mathsf{subst}}^*
\Gamma
$$

On the other hand:
$$
\left\{
\begin{array}{rcl}
	\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C} & \rhd &
	\dbr{\Psi_1}\pairQ x{B}\\
\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}} & \rhd & \dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}
\end{array}
\right\}
\xrightarrow{}_{\mathsf{distr}}^*
\left\{
\begin{array}{rcl}
	\Gamma_1'',
	\dbr{\Psi_{2u}}\bullet\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
	\pairQ x{B}\\
	\Gamma_2'', \dbr{\Psi_{1v}}\bullet\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{y}}} & \rhd &  \br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B} 
\end{array}
\right\}
$$
$$
\xrightarrow{}_{\mathsf{distr}}
\left\{
\begin{array}{rcl}
	\Gamma_1'',
	\dbr{\Psi_{2u}}\br[v]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C''} & \rhd & 
	\pairQ x{B}\\
	\Gamma_2'', \dbr{\Psi_{1v}}\dbr{\Psi_v}\pairQ{v}{D''\ctx{\tensor^\phl{u}}} & \rhd &  \pairQ y{\dual B} 
\end{array}
\right\}
\xrightarrow{}_{\mathsf{subst}}^*
\Gamma
$$


\end{proof}



==> semantics.tex <==
Our next task is to lay the groundwork that will eventually allow us
to establish a semantics for this system via a cut elimination
procedure.
%
% \sonia{the cut rule of linear logic should appear somewhere, either
%   here, or perhaps preferably in the prelim section, to say that it is
%   standard, and it is the case in CP, that semantics is obtained
%   through cut-elimination.}
%  
Adding label to queues and connectives brings along some notational
burden, but it is instrumental to complete the cut-elimination proof.
%
However, this notational overhead comes at a price, since the labels
need to be meticulously maintained: the cut-elimination procedure does
not only simplify the formulas and derivations involved in the cut but
also rewrites the labels used within a sequent.

Elements of a context are formulas which ($i$) feature annotated
connectives and ($ii$) are equipped with queues of messages to be
forwarded; these two new features need to appear in the standard cut
rule of linear logic, and, as a consequence, pose new challenges to
the cut-elimination procedure.
%
A cut rule must cut two elements of a context of the form $\dbr{\Psi_1}\pairQ x A$ and $\dbr{\Psi_2}\pairQ y{\dual A}$.
%
As shown by Proposition~\ref{prop:embed}, in a standard linear logic cut rule, the elements of $\Psi_1$ and $\Psi_2$ would freely occur in the conclusion context as independent formulas. 
%
However, in forwarder logic, they are attached to $\phl x$ and $\phl y$, respectively, and they are the type of messages that must be forwarded. 
%
Hence, after cutting $\pairQ x A$ and $\pairQ y{\dual A}$ we must attach $\Psi_1$ and $\Psi_2$ to other endpoints in the context of the conclusion. 
%
This operation is called \emph{distribution}.

Moreover, since queue elements in the rest of the context are also annotated with endpoints, we must handle those referring  to $\phl x$ and $\phl y$, which are doomed to disappear after the cut. 
%
The \emph{substitution} operation does this guided by the annotations on the cut formulas.
%

%In the following we use $\phl x$ and $\phl y$ for the endpoints that correspond to the two forwarder we wish to cut.
%One of the defining characteristics of a forwarder is that the cut is usually \emph{deep}, which means, the cut-formulas $\pairQ x A$ and $\pairQ y {\dual A}$ occur under a stack of queued messages $\dbr{\Psi_1}$ and $\dbr{\Psi_2}$ respectively.
%In contrast, our cut-elimination for forwarders is compliant with deep cuts. 

Both operations \emph{substitution} and  \emph{distribution} work on a two dimensional depiction of the cut judgements $\Gamma_1, \dbr{\Psi_1}\pairQ xA$ and $\Gamma_2, \dbr{\Psi_2}\pairQ y{\dual A}$ as follows:
\begin{smallequation}\label{eq:cut-pair}
\left\{
\begin{array}{l@{\quad\rhd\quad}l} 
	\Gamma_1 & \dbr{\Psi_1}\pairQ xA\\
	\Gamma_2 & \dbr{\Psi_2}\pairQ y{\dual A}
\end{array}
\right\}
\end{smallequation}
We use the $\rhd$ to single out the cut-formulas and make the rules
that we introduce below more readable. $\rhd$ should not be confused
with derivability in intuitionistic logic.  Moreover, when we need to
single out an operator, for instance to substitute a different name
for its annotation, we use the notation $B\ctx{\tensor^\phl{u}}$, this
indicates the first (leftmost) occurrence of the symbol
$\tensor^{\phl u}$ within proposition $B$.

\begin{example}
	The proposition $B \colonequals(a \tensor b) \tensor^\phl{u} (c \parr d) \tensor^\phl{u} e$ is a well-formed annotated type. 
	%[ ]
	We would write $B\ctx{\tensor^\phl{u}}$ to point to the leftmost occurrence of $\tensor^\phl{u}$.
	%
	Consequently $B\ctx{\tensor^\phl{x}}$ would denote the formula $(a \with b) \tensor^\phl{x} (c \parr d) \tensor^\phl{u} e$.
	%
	On the other hand, $B[\phl x/\phl u]$ would indicate a global substitution of $\phl x$ for $\phl u$, namely the formula
	$(a \tensor b) \tensor^\phl{x} (c \parr d) \tensor^\phl{x} e$.
\end{example}

\mypar{Distribution.}
Given a pair of contexts depicted as in~\eqref{eq:cut-pair},
%\begin{smallequation*}
%\left\{
%\begin{array}{lcl} 
%	\Gamma_1 &\rhd& \dbr{\Psi_1}\pairQ xA\\
%	\Gamma_2 &\rhd& \dbr{\Psi_2}\pairQ y{\dual A}
%\end{array}
%\right\}
%\end{smallequation*}
%
we proceed by distributing each element of the queues $\dbr{\Psi_1}$ and $\dbr{\Psi_2}$ to queues in $\Gamma_2$ and $\Gamma_1$ respectively.
%
Indeed, elements in $\dbr{\Psi_1}$ ($\dbr{\Psi_2}$) have been received at endpoint $\phl x$ ($\phl y$), but when executing the cut $\phl x$ and $\phl y$ disappear and only the other endpoints in $\Gamma_1$ and $\Gamma_2$ remain.
%
Messages in $\Psi_1$ ($\Psi_2$) need now to come from an available endpoint from $\Gamma_2$ ($\Gamma_1$).
%
We always distribute by picking the top element (in our notation
below, a box labelled with $d$) of one of the queues and since the cut
rule is symmetric, we pick from $\Psi_1$.

We start with equipping each queue on the left with a $\bullet$ marker
that ensures that the messages from successive applications of the $\mathsf{distr}$ rule preserve their respective orders.
%
Then, assuming that part of the queues have already been distributed, 
the following is the $\mathsf{distr}$ rewriting that allows us to distribute the top element of the queue in front of endpoint $\phl x$ to endpoint $\phl c$ in $\Gamma_2$
%
%\carsten{FIX: do we need the labels on the distr arrow?}\sonia{I am removing them everywhere}
\begin{smallalign*}
	\left\{
	\begin{array}{l@{\quad\rhd\quad}l}
		\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\tensor^\phl{x}}}  & \br[d]{\pairQ bB}\dbr{\Psi_1}\pairQ{x}{A}
		\\
		\Gamma_2, \dbr{\Psi_{1c}}\bullet\dbr{\Psi_c}\pairQ{c}{C}& \dbr{\Psi_2}\pairQ{y}{\dual A}
	\end{array}
	\right\}
	\xrightarrow{}_{\mathsf{distr}} %\br[d]{\pairQ bB}\circ \phl{c}
	\\
	\left\{
	\begin{array}{l@{\quad\rhd\quad}l}
		\Gamma_1, \dbr{\Psi_{2d}}\bullet\dbr{\Psi_d}\pairQ{d}{D\ctx{\mathbf{\tensor}^\phl{c}}} & \dbr{\Psi_1}\pairQ{x}{A}\\
		\Gamma_2, \dbr{\Psi_{1c}}\br[d]{\pairQ bB}\bullet\dbr{\Psi_c}\pairQ{c}{C} & \dbr{\Psi_2}\pairQ{y}{\dual A}
	\end{array}
	\right\}       
\end{smallalign*}
%
%\noindent
%where the  $\tensor^\phl{x}$ refers to the leftmost occurence of a $\tensor$ labelled with $\phl x$ in proposition $D$.
%



%The distribution rule identifies the connective linked to $x$ in this sequent,  a set of processes $\pairQ {c_i}{C_i}$ in the other sequent, and then redistribute each $\Delta_i$ into their new positions. 

An application  of this rule yields again two sequents.  
%
We move $\br[d]{\pairQ bB}$ from the queue in front of $\pairQ xA$ to endpoint $\phl c$ and the left hand side of $\rhd$ in the top sequent is updated to reflect that $\phl d$ has one fewer communication link with $\phl x$ and communicates with  channel $\phl {c}$ instead, i.e., $\pairQ{d}{D\ctx{\tensor^\phl{x}}}$ becomes $\pairQ{d}{D\ctx{\mathbf{\tensor}^\phl{c}}}$.
%
Eventually, when both queues $\dbr{\Psi_1}$ and $\dbr{\Psi_2}$ have been distributed, the obsolete $\bullet$ markers are removed and the process enters the next phase, substitution. 

Note that the $\mathsf{distr}$ rule is not deterministic, in that the rule does not  uniquely determine, to which endpoint the element  $\br[d]{\pairQ{b}{B}}$ is distributed to.  
%
%This means that differently from standard cut-elimination, the cut-elimination procedure does not rewrite into a unique sequent, but rather a set of possible sequents. 
%
Hence, each application of $\mathsf{distr}$ will determine a particular cut-rule.






\mypar{Substitution.}
After distribution, the cut-formulas are free from their respective
queues which have been placed over endpoints in the rest of the
contexts. The substitution operation is now going to take care of all
those occurrences of $\phl x$ and $\phl y$ in the contexts that still
must disappear by exploiting the annotations on the cut-formula.
%
We start from a configuration of the following form:
\begin{smallequation*}
\left\{
\begin{array}{l@{\quad\rhd\quad}l} 
	\Gamma_1 & \pairQ xA\\
	\Gamma_2 & \pairQ y{\dual A}
\end{array}
\right\}
\end{smallequation*}

The substitution operation is defined inductively following the respective structures of  $\pairQ x{A}$ and $\pairQ y{\dual A}$.  We distinguish three cases, the $\tensor/\parr$ case, the atomic case, and the unit case.

\paragraph{Substitution for $\tensor$ and $\parr$.}
Assume that the cut formulas are of the form
$\pairQ{x}{A \tensor^{\phl{b}} D} $ and
$ \pairQ{y}{\dual A \parr^{\phl{c}} \dual D}$.
%
This enforces that, in the bottom left context ($\Gamma_2$), the endpoint $\phl c$ must always be typed by a proposition that contains a $\tensor^\phl{y}$. The $\phl y$ will need to be substituted by $\tensor^\phl{b}$.
%
In the top left context ($\Gamma_1$) however, there can be two
scenarios: either the endpoint $\phl b$ has an element such as
$\br[\phl{x}] {\pairQ{a}{\dual A}}$ in its queue, i.e.~typed with the
dual of $A$ and that needs to be forwarded to $\phl x$, or it has a
$\parr^\phl{x}$ within its type. In both cases, $\phl x$ needs to be
substituted by $\phl c$.
%

In the first case, 
it gives the following rewriting
%the queue must be relinked to channel $c$ from which $\dual D$ expects to receive the message from
\begin{smallalign*}
	\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1, \br[x] {\pairQ{a}{\dual A}}\dbr{\Psi_b}\pairQ{b}{B} 
	& 
	\pairQ{x}{A \tensor^{\phl{b}} D} 
	\\
	\Gamma_2, \dbr{\Psi_c}\pairQ{c}{C\ctx{\tensor^\phl{y}}} 
	&
	\pairQ{y}{\dual A \parr^{\phl{c}} \dual D} 
\end{array}
\right\}
\xrightarrow{}_{\mathsf{subst}} %\br[c]{\pairQ aA}\circ \phl{b}
\\
\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1, \br[c]{\pairQ{a}\dual{A}}\dbr{\Psi_b}\pairQ{b}{B} 
	& \pairQ{x}{D} \\
	\Gamma_2, \dbr{\Psi_c}\pairQ{c}{C\ctx{\tensor^\phl{b}}}
	&
	\phl y: \thl {D^\perp} 
\end{array}
\right\} 
\end{smallalign*}

In the second case, it gives a similar rewriting  % as $\br[x]{\ldots} \not\in\dbr{\Psi_b}$, 
%we execute the communication in a straighforward way, where the counterparts to $x$ and $y$ are updated by $c$ and $b$, accordingly.

\begin{smallalign*}
	\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1, \dbr{\Psi_b}\pairQ{b}{B\ctx{\parr^\phl{ x}}}  
	& \pairQ{x}{A \tensor^{\phl{ b}} D} \\
	\Gamma_2, \dbr{\Psi_c}\pairQ{c}{C\ctx{\tensor^\phl{y}}}   &
	\pairQ{y}{\dual A \parr^{\phl{ c}} \dual D} 
\end{array}
\right\}
\xrightarrow{}_{\mathsf{subst}}
\\
\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1, \dbr{\Psi_b}\pairQ{b}{B\ctx{\parr^\phl{c}}}  & \pairQ{x}{D} \\
	\Gamma_2,  \dbr{\Psi_c}\pairQ{c}{C\ctx{\tensor^\phl{b}}} &
	\phl y: \thl {D^\perp}
\end{array}
\right\}
\end{smallalign*}


% Identify the type of channel $b$ ($x$) and the topmost element ($y$) in the queue for $c$ and then  record the newly established connection between $b$ and $c$ by replacing  $x$ by $c$ and $y$ by $b$.

\paragraph{Substitution for atoms.}
Substituting atoms is straightforward and completes the substitutions
sequence, by producing the standard judgement.

\begin{smallequation*}
	\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1 & \pairQ{x}{a} \\
	\Gamma_2 & \pairQ{y}{\dual a}
\end{array}
\right\}
\xrightarrow{}_{\mathsf{subst}}
%\left\{
%\begin{array}{c}
	\Gamma_1, \Gamma_2
%\end{array}
%\right\}
\end{smallequation*}

\paragraph{Substitution for units.}
%
Substitution for units resemble the multiplicative connective but with
the added feature of gathering (for a treatment of the multiplicative
connective that includes gathering, see the appendix), but it
terminates the rewriting sequence similarly to the atoms.
%
Assume the cut formulas are $\pairQ{x}{\one^\phl{\tilde a\tilde b}}$ and $\pairQ{y}{\bot^\phl{c}} $.
%
This means that the top context ($\Gamma_1$) can potentially contain some terminated endpoints (here, the $a_i$'s), equipped with a  queue of the form $\dbr{\Psi_{a_i}}\br[x]{\Star}$ and some other channels (here, the $b_j$'s) whose type includes a $\bot^\phl{x}$. These $\phl x$ will need to be substituted by $\phl c$.
%
It also means that the endpoint $\phl c$'s type,  in the bottom context ($\Gamma_2$), embeds a unit $\one$ labelled with a set of endpoints which includes $\phl y$. This $\phl y$ will need to be replaced by the list on endpoints $\phl{\tilde a\tilde b}$.
%
This gives us the following rewriting

\begin{smallalign*}
	\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1,\set[i]{ \dbr{\Psi_{a_i}}\br[x]{\Star}\pairQ{a_i}{\cdot}}, \set[j]{\dbr{\Psi_{b_j}}\pairQ{b_j}{B_j\ctx{\bot^\phl{x}}}}  & 
	\pairQ{x}{\one^\phl{\tilde a\tilde b}}\\
	\Gamma_2,\dbr{\Psi_c}\pairQ{c}{C\ctx{\one^\phl{y\tilde{u}}}} & \pairQ{y}{\bot^\phl{c}} 
\end{array}
\right\}
\xrightarrow{}_{\mathsf{subst}}
\\
\Gamma_1, \set[i]{\dbr{\Psi_{a_i}}\br[c]{\ast}\pairQ{a_i}{\cdot}}, \set[j]{\dbr{\Psi_{b_j}}\pairQ{b_j}{B_j\ctx{\bot^\phl{c}}}},
\Gamma_2,\dbr{\Psi_c}\pairQ{c}{C\ctx{\one^\phl{\tilde a\tilde b\tilde{u}}}}
\end{smallalign*}



In summary, the definition of the cut-rule is a bit more complicated than in classical linear logic: What used to be a simple identification of the cut-formula in the left sequent and its dual on the right, has become a sequence of somewhat cumbersome distribution and substitution steps. Hence, we will show how to adapt the proof accordingly in the rest of this section.

\mypar{Reductive semantics.}
The \cut is defined in terms of distribution and substitution
(applying these rewritings until they come to quiescence) and
represents the interaction between two active processes $\phl P$ and
$\phl Q$.
%
Recall that due to the non-determinism of the $\mathsf{distr}$-rule, each distribution sequence will determine a different conclusion $\Gamma$.
%
%cut-elimination is no longer deterministic or unique.  
%\sonia{no! cut-elimination is deterministic! it is the definition of the cut-rule that is not, but once a cut-rule is used it non-ambiguously determines the conclusion sequent and hence cut-elimination}


\begin{smallequation*}
		\infer[\cut]
	{\phl {\res{xy} (P\pp Q)}\seq^\cut \Gamma}
	{
%		\begin{array}{@{}l} 
			\phl P\seq \Gamma_1, \dbr{\Psi_1}\pairQ xA
%		\quad
& 
		\phl Q\seq\Gamma_2, \dbr{\Psi_2}\pairQ y{A^\perp}
%		 \\[1ex]
%\quad
&
		\big\{\Gamma_1\rhd\dbr{\Psi_1}\pairQ xA,
		\Gamma_2\rhd\dbr{\Psi_2}\pairQ y{\dual
			A}\big\}\rightarrow^*_{\mathsf{distr}}\rightarrow^*_{\mathsf{subst}}\Gamma
%	\end{array}
} 
\end{smallequation*}

We denote by $\phl P \seq^\cut \Gamma$ the fact that a derivation can be constructed using the rules previously introduced for forwarders as well as the additional $\cut$ rule.
%
The rank of a $\cut$ is defined as the size (number of connectives and units) of $A$. 
%
By extension the cut-rank of process $\phl P$ such that $\phl P\seq^\cut\Gamma$, denoted as $\mathtt{rank}(\phl P)$, is the maximum of the ranks of $\cut$ rules occurring in the derivation of this judgement. 

% \begin{remark}
% 	Requiring the queues to be empty would greatly reduce the expressiveness of  forwarders, because this is tantamount to blocking, which is exactly the problem we wish to solve.  If cuts were only allowed at depth $0$, forwarders would just be degenerate processes that are blocked until all messages are successfully forwarded.
% 	\sonia{I don't understand this remark. Remove? Rephrase?}
% \end{remark}




   
As one could hope in the proposition-as-type methodology, semantics of forwarders is obtained through cut-reductions.

\begin{theorem} [Admissibility of \tsc{Cut}]
  Let $\phl P\seq\Gamma_1, \dbr{\Psi_1}\pairQ xA$ and
  $\phl Q\seq\Gamma_2, \dbr{\Psi_2}\pairQ y{A^\perp}$.  
  Then, for
  any $\Gamma$ such that
  $\big\{\Gamma_1\rhd\dbr{\Psi_1}\pairQ xA,\ \Gamma_2\rhd\dbr{\Psi_2}\pairQ y{\dual
    A}\big\}\longrightarrow^*_{\mathsf{distr}}\longrightarrow^*_{\mathsf{subst}}\Gamma$
  there exists $\phl R \seq \Gamma$,
 more precisely, we can define a sequence of reductions $\phl{\res{xy}(P \pp Q)} \reducesto^*_\beta \phl R$ that preserves typing.
\end{theorem}

\begin{figure}[t]
\begin{smallequation*}
		\begin{array}{l@{\qquad}l@{\quad\reducesto_\beta\quad}l}
		(B_1) &
		\phl{\res{xy}(\fwd zx \pp Q)}
		&
		\phl{Q[z/y]}
		\\
		(B_2) &
		\phl{\res {xy}(\close x \pp \wait {y}{Q}  )} 
		&
		\phl{Q^\mathsf{y \leadsto \tilde u}} 
		\\
		(C_1) &
		\phl{\res{xy}(P \pp \wait zQ)}
		&
		\wait{z}{ \phl{\res{xy}(P \pp Q)}}
		\\
		(C_2)
		&
		\phl {\res{xy} (P\pp \recv uvQ)}
		&
		\recv uv{\res {xy}(P\pp Q)} 
		\\
		(C_3) &
		\phl{\res {xy}(P\pp (\send z{v}{Q}{R}))}
		&
		\send zvQ{\res{xy}(P \pp R)}
		\\
		(K) &
		\phl{\res{xy}(\send xa{P}{Q} \pp \recv yc{R}) }
		&
		\phl {\res{xy} (Q\pp \res{a\rhd c} (P\pp R))}
	\end{array}
\end{smallequation*}
	\caption{Cut-reductions for the multiplicative fragment}
	\label{fig:cut-red}
\end{figure}



	We will describe the method of the proof, for the details see the appendix.
	%
	It proceeds by lexicographic induction on the structures of $A$, $\phl P$ and $\phl Q$.
	That is, the induction hypothesis may be applied whenever 
	($i$) the rank of the cut gets smaller,
%	 or ($ii$) the rank stays the same and a $\cuttwo$ is replaced by a $\cut$, 
	or ($ii$) the rank stays the same and the cut is applied to at least one smaller process while the other stays the same.
%	the heights of derivations above the cut is smaller and the other is smaller or stays the same. 

As usual, we can distinguish (B)ase cases, (K)ey cases and (C)ommutative cases, see Figure~\ref{fig:cut-red}. 
%
In the base cases ($B_1$) and ($B_2$), we reach the end of the reduction sequence and the cut disappears all together.
%
In ($B_1$) we replace the cut with a simple uniform substitution; 
in ($B_2$)  on the other hand, we require a non-uniform substitution reproducing the $\mathsf{distr}$ rewriting happening in the original cut.
%
In the commutative cases ($C_1$), ($C_2$) and ($C_3$), the cut is reduced to a cut on $\phl P$ (that remains the same) and on a subprocess of $\phl Q$, to which the induction hypothesis can easily be applied.
%
Identical reductions are of course available symmetrically inverting the roles of $\phl P$ and $\phl Q$.
%
In the key case, the cut is rewritten into a cut of smaller rank on process $\phl Q$ and $\phl S = \phl{\res{a \rhd c}(P \pp R)}$. 
%
This process $\phl S$ is obtained by Lemma~\ref{lem:cuttwo-adm-simp} (see appendix).

The last piece of the puzzle that we need to complete the cut-elimination proof is a property of the distribution/substitution rewriting. 
%
%Intuitively, given a cut on $\pairQ x{A \tensor^u B}$ and $\pairQ y{\dual A \parr^v \dual B}$ concluding in $\Gamma$, it must be possible to follow its structure and reconstruct a shorter reduction, for example starting in $\pairQ x{B}$ and $\pairQ y{\dual B}$ to $\Gamma$, otherwise it will not be possible to apply the induction hypothesis in the cut-elimination proof.  That this is indeed the case guarantees the following inversion lemma, which can be proven by induction on the structure of the rewriting sequence.
%
To ensure that the type of  $\phl {\res{xy} (Q\pp \res{a\rhd c} (P\pp R))}$ is indeed the same as the one of the original process $\phl{\res{xy}(\send xa{P}{Q} \pp \recv yc{R}) }$, we rely on the fact that, if
%
\begin{smallequation*}
	\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1,
	\br[x]{\pairQ{d}{\dual A}}\dbr{\Psi_u}\pairQ{u}{C}  & 
	\dbr{\Psi_1}\pairQ x{A \tensor^\phl{u} B}\\
	\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}} &  \dbr{\Psi_2}\pairQ y{\dual A \parr^\phl{v} \dual B} 
\end{array}
\right\}
\xrightarrow{}_{\mathsf{distr}}^*\xrightarrow{}_{\mathsf{subst}}^*
\Gamma
\end{smallequation*}
%
then there exists a distribution-substitution rewriting sequence such that 
\begin{smallequation*}
	\left\{
\begin{array}{l@{\quad\rhd\quad}l}
	\Gamma_1, \dbr{\Psi_u}\pairQ{u}{C} &
	\dbr{\Psi_1}\pairQ x{B}\\
	\Gamma_2, \dbr{\Psi_v}\pairQ{v}{D\ctx{\tensor^\phl{y}}} &  \dbr{\Psi_2}\br[v]{\pairQ{d}{\dual A}}\pairQ y{\dual B}
\end{array}
\right\}
\xrightarrow{}_{\mathsf{distr}}^*
\xrightarrow{}_{\mathsf{subst}}^*
\Gamma
\end{smallequation*}
%
This can be established by induction over the length of the rewriting sequence.






%
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:
